Fairly Allocating Utility in Constrained Multiwinner Elections

Fairness in multiwinner elections is studied in varying contexts. For instance, diversity of candidates and representation of voters are both separately termed as being fair. A common denominator to ensure fairness across all such contexts is the use of constraints. However, across these contexts, the candidates selected to satisfy the given constraints may systematically lead to unfair outcomes for historically disadvantaged voter populations as the cost of fairness may be borne unequally. Hence, we develop a model to select candidates that satisfy the constraints fairly across voter populations. To do so, the model maps the constrained multiwinner election problem to a problem of fairly allocating indivisible goods. We propose three variants of the model, namely, global, localized, and inter-sectional. Next, we analyze the model's computational complexity, and we present an empirical analysis of the utility traded-off across various settings of our model across the three variants and discuss the impact of Simpson's paradox using synthetic datasets and a dataset of voting at the United Nations. Finally, we discuss the implications of our work for AI and machine learning, especially for studies that use constraints to guarantee fairness.

==> FairlyFairMWE - arXiv-4/new_tex/abstract.tex <==
Fairness in multiwinner elections is studied in varying contexts. For instance, diversity of candidates, representation of voters, or both are separately termed as being fair. A common denominator to ensure fairness across all such contexts is the use of constraints. However, across these contexts, the candidates selected to satisfy the given constraints may systematically lead to unfair outcomes for historically disadvantaged voter populations as the \emph{cost of fairness} may be borne unequally. Hence, we develop a model to select candidates that satisfy the constraints fairly across voter populations. To do so, the model maps the constrained multiwinner election problem to a problem of fairly allocating indivisible goods. We propose three variants of the model, namely, \emph{global}, \emph{localized}, and \emph{inter-sectional}. Next, we analyze the model's computational complexity and present an empirical analysis of the utility traded-off across various settings of our model. 
%across the three variants and 
We observe the potential impact of Simpson's paradox on results using synthetic datasets and a dataset of voting at the United Nations. 
%This implies that a model which is fair for say, African-American Females (intersectionally fair), may not be fair for African-Americans or Females. 
Finally, we discuss the implications of our work on studies that use constraints to guarantee fairness.

%Fairness in multiwinner elections is studied in varying contexts. For instance, diversity of candidates, representation of voters, or both are separately termed as being fair. A common denominator to ensure fairness across all such contexts is the use of constraints. However, across these contexts, the candidates selected to satisfy the given constraints may systematically lead to unfair outcomes for historically disadvantaged voter populations as the \emph{cost of fairness} may be borne unequally. Hence, we develop a model to select candidates that satisfy the constraints fairly across voter populations. To do so, the model maps the constrained multiwinner election problem to a problem of fairly allocating indivisible goods. We propose three variants of the model, namely, \emph{global}, \emph{localized}, and \emph{inter-sectional}. Next, we analyze the model's computational complexity, and we present an empirical analysis of the utility traded-off across various settings of our model across the three variants and discuss the impact of Simpson's paradox using synthetic datasets and a dataset of voting at the United Nations. Finally, we discuss the implications of our work for AI and machine learning, especially for studies that use constraints to guarantee fairness.




% Fairness in multiwinner elections is studied in varying contexts. For instance, diversity of candidates and representation of voters are both separately termed as being fair. A common denominator to ensure fairness across all such contexts is the use of constraints. However, across these contexts, the candidates selected to satisfy the given constraints may systematically lead to unfair outcomes for historically disadvantaged voter populations as the cost of fairness may be borne unequally. 
% Hence, we develop a model to select candidates that satisfy the constraints fairly across 
% voter populations. To do so, the model maps the constrained multiwinner election problem to a problem of fairly allocating indivisible goods. 
% We propose three variants of our model, namely, \emph{global}, \emph{localized}, and \emph{intersectional}.
% %the model to limit the fair allocation to within \emph{similar} populations that share an attribute. 
% Next, we analyze the model's computational complexity, and we present an empirical analysis of the utility traded-off across various settings of our model across the three variants and discuss the impact of Simpson's paradox using synthetic datasets and a dataset of voting at the United Nations.
% Finally, we discuss the implications of our work for AI and machine learning, especially for studies that use constraints to guarantee fairness.

%We discuss the significance of our results for AI and machine learning, including their potential to bolster an emerging paradigm of automated decision making called virtual democracy.







% Fairness in multiwinner elections is studied in varying contexts. For instance, diversity of candidates and representation of voters are both separately termed as being fair. A common denominator to ensure fairness across all such contexts is the use of constraints. However, across these contexts, the candidates selected to satisfy the given constraints may systematically lead to unfair outcomes for historically disadvantaged voter populations. Here, we develop a model that uses various techniques to select candidates that satisfy the constraints fairly across \emph{all} populations. To do so, the model maps the constrained multiwinner election problem to a problem of fairly allocating indivisible goods. We also \emph{localize} the model to limit the fair allocation to within \emph{similar} populations that share an attribute. Finally, we analyze the model's computational complexity and present an empirical analysis of the utility traded-off across various settings of our model.

% Furthermore, the model promisingly makes the constrained multiwinner election hard to manipulate across all the settings. Broadly, our study motivates the need to fairly allocate fairness (globally or locally) in studies that use constraints to guarantee fairness. 


% Fairness in multiwinner elections is studied in varying contexts. For instance, diversity of candidates and representation of voters are both separately termed as being fair. A common denominator across all such contexts is the use of constraints to ensure fairness. However, across all the contexts, the candidates selected to satisfy the given constraints may systematically lead to unfair outcomes for historically disadvantaged voter populations. Here, we develop a model that uses various techniques to select candidates that satisfy the constraints fairly across \emph{all} populations. To do so, the model maps the constrained multiwinner election problem to a problem of fairly allocating indivisible goods. We also \emph{localize} the model to limit the fair allocation to within \emph{similar} populations. Finally, we analyze the model's computational complexity and 
% %Though the model is generally intractable, it is tractable under realistic settings. 
% %Finally, we 
% present an empirical analysis of the utility traded-off across various settings of our model.  

% Furthermore, the model promisingly makes the constrained multiwinner election hard to manipulate across all the settings. Broadly, our study motivates the need to fairly allocate fairness (globally or locally) in studies that use constraints to guarantee fairness. 




% Fairness in multiwinner elections is studied in varying contexts. A common denominator is the use of constraints to ensure fairness. However, the candidates selected to satisfy the given constraints may systematically lead to unfair outcomes for historically disadvantaged voter populations. Here, we develop a model that proposes various techniques to select candidates to satisfy constraints. Specifically, ..... We study our model theoretically and empirically. Broadly, our study .....
  

% % Fairness has recently received particular attention from the computer science research community. However, fairness comes at a cost as it may lead to, for instance, a drop in accuracy of machine learning classifiers or a drop in utility of the winning committee selected in multiwinner elections. This cost may be disproportionately borne by historically disadvantaged groups, and such unfairness may be experienced by multiple/different actors of the system. For example, enforcing diversity among candidates in a multiwinner election may lead to a greater decrease in representation for one voter population than the other. This is to say that the cost to include females in a committee may be borne by female voters more than the male voters
% % %\footnote{We limit our example to genders assigned at birth for ease of understanding. The unfairness may hold for any gender that a person may identify with.}
% % .

% Fairness has recently received particular attention from the computer science research community. However, fairness comes at a cost. For instance, it may lead to a drop in the accuracy of a machine learning classifier or a drop in the utility of the winning committee selected in a multiwinner election. This cost may be disproportionately borne by historically disadvantaged groups and such unfairness may be experienced by different actors of the system. For example, enforcing diversity among candidates in a multiwinner election may lead to a greater decrease in the representation for one voter population than the other. It implies that the cost to include female candidates in a committee may be borne by female voters more than male voters.




% % In this paper, we study this phenomenon of unfairness through fairness in the context of multiwinner elections. We introduce a novel model that maps the diverse and representative multiwinner election problem to a problem of fairly allocating indivisible goods. This helps to balance the loss in utility across candidate groups and voter populations. We analyze the model's computational complexity and present an empirical analysis of the running time and the balance in utility traded-off across various setting of our model.
% % Overall, our work motivates that any study on fairness should systematically assess \emph{who} pays \emph{what} cost to achieve fairness, and then mitigate unintended unfairness caused through fairness.



% In this paper, we study this phenomenon of unfairness through fairness in the context of multiwinner elections. We introduce a novel model that maps the diverse and representative multiwinner election problem to a problem of fairly allocating indivisible goods. This helps to balance the loss in utility across candidate groups and voter populations. We analyze the model's computational complexity and present an empirical analysis of the balance in utility traded-off across various settings of our model. 
% Overall, our work motivates that any study on fairness should systematically assess \emph{who} pays \emph{what} cost to achieve fairness and then mitigate unintended unfairness caused through fairness.

==> FairlyFairMWE - arXiv-4/new_tex/complexity.tex <==
\section{Complexity Results}
\label{sec:complexity}

In this section, we analyze the computational complexity of various settings of our global fair allocation model. 

Note that global fair allocation is a generalization of localized fair allocation. Hence, a polynomial-time algorithm we give for the former holds for the latter (but with trivial modification). On the other hand, the NP-hardness of the localized fair allocation implies the NP-hardness of the global fair allocation but not vice versa. Hence, we design each NP-hardness reduction for global fair allocation such that it holds for localized and inter-sectional fair allocation as well.


\subsection{FEC} 

We first present a polynomial-time algorithm for Favorite-Envyfree-Committee (FEC), FEC up to $k-1$, and FEC up to $k-2$.

\begin{theorem}\label{thm:FECuptoxP}
Given a winning \DIRE Committee $W$ and an integer $x$ in $\{0,$ $k-2,$ $k-1\}$, there is a polynomial time algorithm that determines whether a FEC up to $x$, W', exists such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$.
\end{theorem}

\begin{algorithm}[t!]
\caption{FEC Algorithm}
\label{alg:algorithmFEC}
\begin{flushleft}
\textbf{Input}:\\
$W_P$, $\forall P \in \mathcal{P}$ - winning committee of each population\\
$l_P^R$, $\forall P \in \mathcal{P}$ - diversity constraints\\
$l_G^D$, $\forall G \in \mathcal{G}$ - representation constraints\\
$W$ - Winning \DIRE Committee\\
\textbf{Output}: True if FEC exists, False otherwise\\
\end{flushleft}
%When $x=0$:
\begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=0$}
\STATE $S$ = $\bigcup {c\in C}: \forall P \in \mathcal{P},$ $ \max_{c \in W_P} \mathtt{f}_{\Borda}^{W_P}(c)$

\STATE \textbf{if} $|S|>k$ \textbf{then} \textbf{return} {False}
\STATE \textbf{if} $S\subseteq W$ and  $|S|>0$ \textbf{then} \textbf{return} {True}
\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \cap S|<l_G^D$ \textbf{then} \textbf{return} {False}
\ENDFOR
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $|W_P \cap S|<l_P^R$ \textbf{then} \textbf{return} {False}
\ENDFOR
\STATE \textbf{return} {True}
\ENDIF
% \end{algorithmic}
% %When $x= k-1$:
% \begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=k-1$}
\STATE \textbf{return} {True}
\ENDIF
% \end{algorithmic}
% %When $x=k-2$:
% \begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=k-2$}
\STATE $S$ = $\phi$

\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE $S$ = $W \setminus$ $\{\forall c \in W_P : c$ is the lowest scoring candidate $\mathtt{f}_{\Borda}^{W_P}(c)$ among $W_P\}$
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $|W_P \cap S|<l_P^R$ \textbf{then} \textbf{return} {False}
\ENDFOR

\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \cap S|<l_G^D$ \textbf{then} \textbf{return} {False}
\ENDFOR
\ENDFOR
\STATE \textbf{return} {True}
\ENDIF
\end{algorithmic}
\end{algorithm}


\begin{proof}
Algorithm~\ref{alg:algorithmFEC} runs in time polynomial of the size of the input. For correctness, consider the following cases:

\begin{itemize}
    \item \textbf{When $\mathbf{x=0}$}, FEC up to 0 can only exist if $\forall P \in \mathcal{P}$, the population top-scoring candidate $\mathtt{f}_{\Borda}^{W_P}(c)$ is in the committee. Hence, we select each and every top-ranked candidate into set $S$. Then, if set $S$ satisfies all the given constraints, then we know FEC up to 0 exists.
    \item \textbf{When $\mathbf{x=k-1}$}, then the existence of a \DiRe committee implies the existence of FEC as FEC up to $k-1$ is equivalent to satisfying the requirement that each population has at least one candidate in the committee, which is in line with the definition of the \DiRe committees.
    \item \textbf{When $\mathbf{x=k-2}$}, we iterate over each population $P \in \mathcal{P}$ such that we remove the population's winning committee's $W_P$ least favorite candidate. If the candidates that remain in $W$ satisfy all the constraints after the removal of this candidate, then it implies that FEC up to $k-2$ exists. This is because if a \DiRe committee exists even after removing a population's least favorite candidate, then it implies that FEC up to $k-2$ also exists. 
\end{itemize}

\end{proof}

We now present hardness\footnote{The hardness results throughout the paper are under the assumption P $\neq$ NP.} results and differ the proofs to the appendix. 

\begin{theorem}\label{thm:FECuptoxNP-hard}
Given a \DIRE Committee $W$ and an integer $x$ in $[1,$ $k-3]$, it is NP-hard to determine whether a FEC up to $x$, W', exists such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$, even when  $l^D_G=0$ and $l^R_P=0$.
\end{theorem}






\subsection{UEC} A Utility-Envyfree-Committee (UEC) is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) = 0 \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| = 0 \]

%\vspace{0.2cm}
\begin{theorem}\label{thm:UECNP-hard}
Given a \DIRE Committee $W$, it is NP-hard to determine whether a UEC, $W'$, exists such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$, even when $l^D_G=0$ and $l^R_P=0$.
\end{theorem}



The hardness of UEC up to $\eta$ follows from the hardness of UEC.
%\vspace{0.1cm}
\begin{corollary}\label{thm:UECuptoetaNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a UEC up to $\eta$, for all $\eta$ in $\mathbb{Z}$ such that $\eta$ in $[0,$ $\frac{(m-1)\cdot(m)}{2})$, exists such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$.
\end{corollary}


Note that when $\eta=0$, UEC up to $\eta$ and UEC are equivalent. When $\eta=\frac{(m-1)\cdot(m)}{2}$, UEC up to $\eta$ and \DiRe committee are equivalent.
    
\subsection{WEC} A Weighted-Envyfree-Committee (WEC) is a $k$-sized committee such that it aims to

%\[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|) \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| = 0 \]


%\vspace{0.1cm}
\begin{theorem}\label{thm:WECNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether a WEC, $W'$, exists such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$, even when $l^D_G=0$ and $l^R_P=0$.
\end{theorem}




The hardness of WEC up to $\zeta$ follows from the hardness of WEC.

\begin{corollary}\label{thm:WECuptozetaNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a WEC up to $\zeta$, for all $\zeta$ in $\mathbb{Q}$ such that $\zeta$ in $[0,$ $1)$, exists such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$.
\end{corollary}



Note that when $\zeta=0$, WEC up to $\zeta$ and WEC are equivalent. When $\zeta=1$, WEC up to $\zeta$ and \DiRe committee are equivalent.

% \section{Mitigating Manipulation in \DIRE Elections}

% Another unintended consequence and cause of unfairness in \DiRe committees is that it easily allows manipulation\footnote{
% All voting mechanisms are known to be susceptible to manipulation \cite{gibbard1973manipulation}, i.e., a situation when a strategizing voter or a group of voters misrepresents his preferences in order to obtain a more desirable outcome. See \cite{elkind2005hybrid} for details.} of outcomes by larger populations to adversely impact the smaller, under-represented populations. For example, assume Californian voters in Figure~\ref{fig:whatexample/voters} are already manipulated. This is to say that had the California voters \emph{not} swapped positions of $c_5$ and $c_6$, then Illinois' most preferred candidate $c_5$ would have been part of the \DiRe committee implicitly. However, the votes are manipulated by changing the preferences among the non-top-$k$ candidates preferred by the Californian voters. This resulted in an adverse outcome for Illinois, without affecting California (see Example~\ref{eg-balanced}).  

% \begin{theorem}\label{thm:DiReManipulation-easy}
% If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then there is a polynomial time algorithm that can either help some manipulator population $P \in \mathcal{P}$ manipulate \DiReCWD or determine that \DiReCWD is not manipulable as long as the population $P$ satisfies the following conditions:
% \begin{itemize}
%     \item $|P|>|P'|$, for all $P' \in \mathcal{P}$ such that $P \neq P'$ 
%     \item $P$ swaps preferences within $C \setminus W_P$
% \end{itemize}
% \end{theorem}

% \begin{algorithm}[t!]
% \caption{\DiReCWD Manipulation Algorithm}
% \label{alg:algorithmManipulation}
% \begin{flushleft}
% \textbf{Input}:\\
% $W_P$, $\forall P \in \mathcal{P}$ - winning committee of each population\\
% $l_P^R$, $\forall P \in \mathcal{P}$ - diversity constraints\\
% $l_G^D$, $\forall G \in \mathcal{G}$ - representation constraints\\
% $W$ - Winning \DIRE Committee\\
% \textbf{Output}: Manipulated votes if manipulation possible, False otherwise\\
% \end{flushleft}

% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE $P_{\max}$ = $P \in \mathcal{P}:\max(|P|)$
% \STATE $E_{\text{actual}}$ = Store the actual votes and $W_P$, $\forall P \in \mathcal{P}$ of election $E$

% \FOR{\textbf{each} $c \in C \setminus W_{P_{\max}}$}
% \FOR{\textbf{each} $c' \in C \setminus W_{P_{\max}} \setminus c$}
% \STATE swap $\pos_v(c)$ and $\pos_v(c')$ for all $v\in P_{\max}$
% \STATE $E_{\text{manip}}$ = Store the manipulated votes and corresponding $W_P$,  $\forall P \in \mathcal{P}$ of election $E$
% \FOR{\textbf{each} $P \in \mathcal{P}$}
% \STATE \textbf{if} $W_P \in E_{\text{actual}} \neq W_P \in E_{\text{manip}}$ and $|W_P \in E_{\text{manip}} \cap W\in E_{\text{manip}}|<l_P^R$ \textbf{then} \textbf{return} Maipulated Election $E_{\text{manip}}$
% \ENDFOR
% \FOR{\textbf{each} $G \in \mathcal{G}$}
% \STATE \textbf{if} $|G \in E_{\text{manip}} \cap W\in E_{\text{manip}}|<l_G^D$ \textbf{then} \textbf{return} Maipulated Election $E_{\text{manip}}$
% \ENDFOR
% \STATE swap $\pos_v(c)$ and $\pos_v(c')$ for all $v\in P_{\max}$
% \ENDFOR
% \ENDFOR
% \STATE \textbf{return} {False}
% \end{algorithmic}
% \end{algorithm}
% \begin{proof}
% Algorithm~\ref{alg:algorithmManipulation} clearly runs in time polynomial of the size of input. Note that as $\mathtt{f}$ is a monotone, separable scoring function, we know that 
% \[\mathtt{f}(W)=\sum_{c\in W}\mathtt{f}(c)\] 
% Hence, it implies that computing $W_P$, $\forall P \in \mathcal{P}$ and $W$ for each of the manipulated instances of the election takes polynomial time. For correctness, it is easy to see that the largest population exhaustively swaps each of its bottom $m-k$ candidates and compares the change in outcome. If the outcome changes for any other population or candidate group, then manipulation is successful. Otherwise, the algorithm terminates by returning False.

% Note that the algorithm can be easily modified to assess if \emph{any} population can manipulate the election. Instead of choosing the largest population in Line 1 of the algorithm, we can have a For loop that iterates over each population and checks whether they can manipulate the result or not.
% \end{proof}


% For the last theorem, note that the NP-hardness of finding a \DiRe committee does \emph{not} follow and result in NP-hardness of manipulating \DiRe committee elections. This is because we assume that a \DiRe committee is given as input. In contrast, the next three proofs show that even when \DiRe committees are given, using FEC, UEC, or WEC makes it hard to manipulate \DiRe committee elections. Thus, the models proposed in this paper also mitigate an unintended consequence of imparting fairness (enforcing constraints) in elections, the consequence being the ease to manipulate elections.

\begin{figure*}[t!]
\centering
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm]{new_figures/fav-envyfree-proportion.pdf}
  \caption{\textbf{FEC violated}}
  \label{fig:fec/proportion}
\end{subfigure}%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm]{new_figures/utility-envyfree-proportion.pdf}
  \caption{\textbf{WEC violated}}
  \label{fig:wec/proportion}
\end{subfigure}%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth, trim=0 0cm 0cm 0cm]{new_figures/fav-envyfree-utility.pdf}
  \caption{\textbf{Loss in utility- FEC}}
  \label{fig:fec/utility}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth, trim=0 0cm 0cm 0cm]{new_figures/utility-envyfree-utility.pdf}
  \caption{\textbf{Loss in utility - WEC}}
  \label{fig:wec/utility}
\end{subfigure}

\caption{The proportion of the population who are envious of at least one other population based on the criteria of (a) favorite-envyfreeness (FEC) and (b) weighted-envyfreeness (WEC). The loss in utility, in terms of the ratio of the utility of (c) FEC committee vs optimal \DiRe committee, to achieve FEC, whenever possible and (d) WEC committee vs optimal \DiRe committee, to achieve WEC, whenever possible. Each selection of $\pi$ (\# voter attributes) has 5 instances generated using \textbf{SynData1}.}
\label{fig:fec}
\end{figure*}

% Promisingly, our model has an advantage as even the easiest version of each of the envyfreeness models makes the \DiRe committee selection problem resistant to manipulation. This holds for the localized fair allocation model as well. In principle, this is because swapping non-top-$k$ preferences by Californian voters penalizes them as well. 



% \begin{corollary}\label{thm:DiReManipulationFEC-hard}
% If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a FEC, such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$.
% \end{corollary}

% \begin{proof}
% Theorem~\ref{thm:FECuptoxNP-hard} showed that finding an FEC is NP-hard. Hence, if finding FEC in a regular election is NP-hard, then the hardness of manipulating an FEC election follows the hardness of finding an FEC.
% \end{proof}
% %\vspace{0.1cm}
% \begin{corollary}\label{thm:DiReManipulationUEC-hard}
% If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a UEC, such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$.
% \end{corollary}
% \begin{proof}
% Theorem~\ref{thm:UECNP-hard} showed that finding a UEC is NP-hard. Hence, if finding UEC in a regular election is NP-hard, then the hardness of manipulating a UEC election follows the hardness of finding a UEC.
% \end{proof}
% %\vspace{0.1cm}
% \begin{corollary}\label{thm:DiReManipulationWEC-hard}
% If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a WEC, such that for all candidate groups $G$ in $\mathcal{G}$, the diversity constraint $l^D_G \leq |G \cap W'|$ and for all voter populations $P$ in $\mathcal{P}$, the representation constraint $l^R_P \leq |W_P \cap W'|$.
% \end{corollary}

% \begin{proof}
% Theorem~\ref{thm:WECNP-hard} showed that finding a WEC is NP-hard. Hence, if finding WEC in a regular election is NP-hard, then the hardness of manipulating a WEC election follows the hardness of finding a WEC.
% \end{proof}

% In summary, while mitigating utility-based unfairness caused due to fairness is generally hard, our models make causing manipulation-based unfairness hard as well. The latter intractability is desirable.

% %In summary, we deem these proposed notions of envyfreeness among voter populations to be of interest, especially due to the promising empirical results that we got from our initial analysis (discussed in the next section). We also plan to study the theoretical aspects of these notions.

==> FairlyFairMWE - arXiv-4/new_tex/conc.tex <==
%\vspace{-0.25cm}
\section{Conclusion and Future Work}
\label{sec:conc}
%\vspace{-0.1cm}



Our work motivates the need to fairly allocate utility in constrained multiwinner elections. 
%This can be achieved by systemically analyzing \emph{who} pays \emph{what} cost to achieve fairness. 
Such analysis should also be carried out for all the actors of any system that guarantees fairness through the use of constraints. Application includes in domains such as machine learning \cite{golz2019paradoxes} and recommender systems \cite{zehlike2022fairness}.   
%In summary, we showed that just like it is important to ensure that the cost to include female candidates in a committee should not be borne by female voters more than male voters, any machine learning model that makes decisions affecting humans should ensure that introducing fairness does not cause unfairness due to change in other aspects of the model. 
Next, on the technical front, we did an extensive complexity analysis. While the hardness results in the paper may seem negative, 
%we stress that these results provide an important foundation for future work in this domain. For example, 
we expect committee size to be small in the real world. Hence, all our hardness results trivially become (fixed-parameter) tractable. 



% We showed that any paper that works on fairness should 
% \begin{itemize}
%     \item we operationalized a model that mitigates unfairness caused through fairness
%     \item 
% \end{itemize}

% With diversity in multiwinner elections becoming necessary, we showed that \textbf{only diversity can do more harm than good} as the cost of diversity may disproportionately be paid more by historically under-represented voter population. Hence, we developed \DiReCWD model, which enforces diversity \textbf{and} representation constraints.
% %we motivated the need for diversity \textbf{and} representation constraints, and developed \DiReCWD model. 
% We studied its computational properties theoretically and empirically. %which gives DiRe committees. 
% %Our model is needed as the call for diversity is becoming ubiquitous. 
% %However, \textbf{only diversity can do more harm than good} as the cost of diversity may disproportionately be paid more by historically disadvantaged population. 
% We also delineate the candidate and voter attributes even when they coincide as we observed that \textbf{diversity does not imply representation and vice versa}, which contrasts the common understanding, and hence, requires further investigation.  %mhaving a female candidate on the committee is different from having a candidate on the committee who is preferred by the female voters, and who themselves may or may not be female. These two are separate but equally important aims that need to be achieved simultaneously.


%\julia{In this section I'm missing what you actually propose to do.  Study the feasibility or also develop algorithms to identify committees?  If the latter, then what algorithmic techniques seem promising to you?  Please add a section explaining what you actually propose to accomplish.  Otherwise it's not clear what the experimental evaluation is for, for example.}

% In the previous sections, we presented our preliminary work on introducing different methods to answer  \emph{what} candidates to choose for a well-rounded story on fairness in multiwinner elections. More specifically, we defined multiple methods to quantify envyfreeness among voter populations and did an initial empirical study to evaluate the feasibility of an envyfree committee and if feasible, the drop in utility caused by the introduction of this new answer on fairness. Building on the promising initial results that showed feasibility of envyfree committees and at a small drop in the utility, we will develop a framework to better understand our notion, both theoretically and empirically.

% \begin{itemize}
    % \item \textbf{Theoretical:} We plan to relax each of the envyfree definitions we proposed in Section~\kunal{sec:what/intro}, namely, Favorite-Envyfree Committee (FEC), Utility-Envyfree Committee (UEC), and Weighted-Envyfree Committee (WEC). We are motivated to do so by the literature on fair resource allocation \cite{brandt2016handbook} that relaxes the idea of envyfree resource allocation to envyfree resource allocation except one and envyfree resource allocation except cheapest. Finally, in line with previous work that showed an envyfree resource allocation except one always exists under monotonicity, we plan to give similar guarantees on existence of FEC, UEC, WEC and their relaxed variants. 
    
    % \item \textbf{Algorithmic:} We plan to study the computational complexity of finding a committee under each setting of envyfreeness. We expect the problem to be NP-hard, and if so, we plan to provide approximation and parameterized complexity results, assuming we are given DiRe committees, which satisfy all the diversity and representation constraints, as input. We can continue on this path even if we find efficient ways to solve the DiRe committee winner determination problem. Overall, we plan to show the best possible approximation ratios we can get. We will also study the hardness of approximation (inapproximability) to understand the ratio limits up to which one can hope to design efficient algorithms. We will also give the parameters, which when fixed, can solve our problem efficiently.
    
    % Alternately, if DiRe committees are not given as input and if we do not find any efficient way to find the DiRe committees, then a more practical approach is to may be formulate our problem of finding a committee under each setting of envyfreeness that satisfy the diversity and representation constraints as integer programs. We note that even finding a feasible DiRe committee is usually NP-hard (\DiReCF results, Section~\kunal{add}). Therefore, we cannot not expect to solve our problem in time polynomial in the size of input. Next, if we do not find any efficient way to find the DiRe committees, then we do not expect to find efficient approximation or parameterized complexity results for our problem either. Hence, formulating our problem as integer programs may be the best choice. We note that standard integer programming platforms like Gurobi \cite{gurobi2018gurobi} allow us to solve reasonably large instances in a very small amount of time, thus the worst-case exponential time required in the worst case is not an issue.
    
%     \item \textbf{Empirical:} As done in Section~\ref{sec:what/empres}, our empirical analysis will continue to focus on understanding the proportion of populations that are envyfree across various settings. Next, if committee(s) that makes populations envyfree exists, we will analyze the cost of utility paid to find this envyfree committee.
% \end{itemize}

==> FairlyFairMWE - arXiv-4/new_tex/empirical.tex <==




\section{Empirical Analysis}
\label{sec:what/empres}



We empirically assess the effect of having each version of the envyfree committee on the utility of the winning committee across different scoring rules.% using synthetic datasets. 

\subsection{Datasets and Setup}
\label{sec:empres/data}
%\subsubsection{Real Datasets}

% \vspace{-.15cm} \paragraph{RealData 1:} The \emph{\underline{Eurovision}} dataset \cite{Kaggle2019Eurovision} consists of 26 countries ranking the songs performed by each of the 10 finalist countries. 
% %While the contest aims to select a single winner, 
% We aim to select a 5-sized DiRe committee. Each candidate %a song performed by a country, 
% has two attributes, the European region and the language of the song performed. Each voter has one attribute, the country's European region. %Specifically for the European region attribute, Australia and Israel were labeled as ``Others'' as they are not a part of Europe.

%\vspace{-.15cm} 
\paragraph{RealData 1:} The \emph{\underline{United Nations Resolutions}} dataset \cite{DVN/LEJUQZ_2009} consists of 193 UN member countries 
%of the world 
voting for 1681 resolutions presented in the UN General Assembly from 2000 to 2020. For each year, we aim to select a 12-sized \DiRe committee. Each candidate has two attributes, the topic of the resolution and whether a resolution was a significant vote or not. Each voter has one attribute, the continent.

%\vspace{-.15cm} 
\paragraph{SynData 1:} We set committee size ($k$) to 6 for 100 voters and 50 candidates. We generate complete preferences using RSM by setting selection probability $\Pi_{i, j}$ to replicate Mallows' \cite{Mallows1957} model ($\phi=0.5$, randomly chosen reference ranking $\sigma$ of size $m$) (Theorem 3, \cite{chakraborty2020algorithmic}) and preference probability $p(i)=1$, $\forall i \in [m]$. We randomly divide the candidates and voters into groups and populations, respectively.%, to get a total order.

 %A higher number of divisions would be infeasible. % 
%as allowing unrealistically high number of groups and populations resulted in infeasible committee, even for $\mu=\pi=1$. 

%\vspace{-.15cm} 
\paragraph{SynData 2:} We use the same setting as SynData 1, except we fix $\mu$ and $\pi$ each to 2 and vary the cohesiveness of voters by setting selection probability $\Pi_{i, j}$ to replicate Mallows' \cite{Mallows1957} model's $\phi$ $\in$ $[0.1$, $1]$, with increments of 0.1.  We divide the candidates into groups and voters into populations in line with \textbf{SynData 1}.


















% \subsection{Setup}
% \label{sec:empres/setup}

\paragraph{System.}
%Experiments to assess the efficiency of our algorithm were carried out in 
 %We believe this to be a move towards a more equitable infrastructure for computing as not all researchers may have access to funds to use a commercial solver. 
We used a controlled virtual environment using Docker(R) on a 2.2 GHz 6-Core Intel(R) Core i7 Macbook Pro(R) @ 2.2GHz with 16 GB of RAM running macOS Big Sur (v11.1). %Our code can run on a less state-of-the-art machine as well. 
We used Python 3.7. Note that we used a personal machine without requiring any commercial tools.

\paragraph{Constraints.}
For each $G \in \mathcal{G}$, 
%set the upper constraint $u_G^D=min(k,|G|)$ and 
we choose $l_G^D = 1$. For each $P \in \mathcal{P}$, 
%set $u_P^R = k$ and 
we choose $l_P^R = \min(1,$ $k \cdot \frac{|P|}{n})$. Thus, each population is guaranteed at least one member, even if their size is small.


\paragraph{Voting Rules.} We use $k$-Borda and $\beta$-CC.


\paragraph{Metrics.} 
We use two metrics: (i) we compute the ratio of utilities of an envyfree committee to an optimal \DiRe committee. A higher ratio is desirable as it means a lesser difference between the two utilities. (ii) we measure the mean of the minimum proportion of populations that always remain envious in the case of FEC and the mean of the maximum difference in utilities that always remain between optimal \DiRe committee and UEC (or WEC).




















% \begin{figure}[t!]
% \centering
% \begin{subfigure}{.23\textwidth}
%   \centering
%   \includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm]{new_figures/fav-envyfree-proportion.pdf}
%   \caption{\textbf{proportion of FEC violated}}
%   \label{fig:fec/proportion}
% \end{subfigure}%
% \begin{subfigure}{.23\textwidth}
%   \centering
%   \includegraphics[width=\linewidth, trim=0 0cm 0cm 0cm]{new_figures/fav-envyfree-utility.pdf}
%   \caption{\textbf{Loss in utility}}
%   \label{fig:fec/utility}
% \end{subfigure}

% \caption{(a) The proportion of population who are envy of at least one other population based on the criteria of favorite-envyfreeness (FEC). (b) The loss in utility, in terms of the ratio of utility of FEC committee vs optimal DiRe committee, to achieve FEC, whenever possible. Each selection of $\pi$ (\# voter attributes) has 5 instances.}
% \label{fig:fec}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \begin{subfigure}{.23\textwidth}
%   \centering
%   \includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm]{new_figures/utility-envyfree-proportion.pdf}
%   \caption{\textbf{WEC violated}}
%   \label{fig:wec/proportion}
% \end{subfigure}%
% \begin{subfigure}{.23\textwidth}
%   \centering
%   \includegraphics[width=\linewidth, trim=0 0cm 0cm 0cm]{new_figures/utility-envyfree-utility.pdf}
%   \caption{\textbf{Loss in utility}}
%   \label{fig:wec/utility}
% \end{subfigure}

% \caption{(a) The proportion of population who are envy of at least one other population based on the criteria of weighted-envyfreeness (WEC). (b) The loss in utility, in terms of the ratio of utility of WEC committee vs optimal DiRe committee, to achieve WEC, whenever possible. Each selection of $\pi$ (\# voter attributes) has 5 instances.}
% \label{fig:wec}
% \end{figure}

\subsection{Results}

\subsubsection{Using SynData1}

%\paragraph{Favorite-Envyfree Committee (FEC)} 
\paragraph{FEC.} We found that the proportion of populations that are envious increases with an increase in the number of attributes (Figure~\ref{fig:fec/proportion}). Interestingly, we observed that an optimal \DiRe committee found using the $\beta$-CC rule was also FEC whenever the number of populations $|\mathcal{P}|$ was less than committee size $k$. A similar observation didn't hold for $k$-Borda. Similarly, the loss in utility (Figure~\ref{fig:fec/utility}) when using $\beta$-CC was lower than $k$-Borda. We note that loss in utility is inversely proportional to the utility ratio. Both these observations can be attributed to $\beta$-CC's design that ensures proportional representation. 



%We propose to study a natural relaxation to Favorite-Envyfree Committee (FEC), the Favorite-Envyfree Committee except $x$ where $x$ is the number of positions for which a population is envyfree. Specifically, a population is envyfree if any candidate up to their $x$-most preferred candidate is in the committee. 

%\paragraph{Utility-Envyfree Committee (UEC)}
\paragraph{UEC.} We found the proportion of populations that are not envyfree to be consistently $\geq 93\%$ for all instances, starting from voters having just one attribute. Thus, measuring the loss in utility is also not possible. This can be attributed to the strict requirement of each population having equal utility from the committee. %We propose to relax UEC by using UEC except $y$, where a population is envyfree if the difference in the utility that the population gets from the winning committee is within $y$ points of all other populations. 



%\paragraph{Weighted-Envyfree Committee (WEC)}
\paragraph{WEC.} This metric provided the best results. While we report similar observations as that for FEC, we note a significant drop in the proportion of populations that are envious (Figure~\ref{fig:wec/proportion}) and a significant rise in the utility ratio (Figure~\ref{fig:wec/utility}), meaning the loss in utility decreased significantly to up to 15\% only. 



% \item \textbf{Empirical:} As done in Section~\ref{sec:what/empres}, our empirical analysis will continue to focus on understanding the proportion of populations that are envyfree across various settings. Next, if committee(s) that makes populations envyfree exists, we will analyze the cost of utility paid to find this envyfree committee.


\subsubsection{Using SynData2}
\paragraph{FEC.} We found that the proportion of populations that are envious decreases with an increase in the cohesiveness of voters (Figure~\ref{fig:fec/proportionphi}).  Similarly, the loss in utility (Figure~\ref{fig:fec/utilityphi}) when using $\beta$-CC was lower when voters were less cohesive and higher when more cohesive. We note that loss in utility is inversely proportional to cohesiveness. 



%We propose to study a natural relaxation to Favorite-Envyfree Committee (FEC), the Favorite-Envyfree Committee except $x$ where $x$ is the number of positions for which a population is envyfree. Specifically, a population is envyfree if any candidate up to their $x$-most preferred candidate is in the committee. 

\paragraph{UEC.} The proportion of populations that are not envyfree to be consistently $\geq 89\%$ for all instances, starting from voters having no cohesiveness. Thus, measuring the loss in utility is also not possible. In line with our observation previously, this can be attributed to the strict requirement of each population having equal utility from the committee. For $\eta$ relaxation as well, our previous observation of relaxation holds as UEC is better than the relaxation of FEC.%%We propose to relax UEC by using UEC except $y$, where a population is envyfree if the difference in the utility that the population gets from the winning committee is within $y$ points of all other populations. 

\paragraph{WEC.} This metric again provided the best results. We report similar observations as that for FEC. Promisingly, there was a rise in the utility ratio (Figure~\ref{fig:wec/utilityphi}) but a drop in the proportion of populations that are envious (Figure~\ref{fig:wec/proportionphi}). Overall, when compared to FEC, WEC turns out to be a better metric. Also, consistent with observations made for FEC, the proportion of envious populations decreased with an increase in cohesiveness and the drop utility ratio also decreased with an increase in cohesiveness. Finally, we found that the proportion of populations that are envious decreases with an increase in $\zeta$ (WEC up to $\zeta$). The decrease was steeper when $\phi$ was low (mean rate of decrease 1.5\% per $\zeta$ for $\phi=0.0$ to 0.1\% per $\zeta$ for $\pi=0.8$).

\subsubsection{Localized Fair Allocation}
Localized fair allocation was easier to satisfy as compared to global fair allocation. This observation, as expected, was coherent across both the datasets, all the three envyfreeness techniques, and their corresponding relaxations. The mean utility ratio for the non-relaxed techniques was significantly higher (94\% vs 85\% for global fair allocation). Specifically, the mean utility ratio was much higher for SynData2 vs SynData1 (98\% vs 92\%). Interestingly, there was no statistically significant relationship between the utility ratio and the mean number of population per attribute (Pearson's correlation, $r=-0.85$, $p>0.05$). This can be because of the varying number of attributes that the dataset has.

\subsubsection{Inter-sectional Fair Allocation and Simpson's Paradox}
Inter-sectional fair allocation was almost as difficult to satisfy as compared to global fair allocation. This observation was coherent across both the datasets, all the three envyfreeness techniques, and their corresponding relaxations. However, an interesting observation was the presence of instances that were not globally fairly allocated but were inter-sectionally fairly allocated. For example, a committee that was not fairly allocated between, say, females and African-Americans was fairly allocated to African-American females. We attribute this observation to Simpson's paradox. The proportion of instances where we observed the presence of Simpson's paradox was 14.8\%. %The mean utility ratio for the non-relaxed techniques was significantly higher (94\% vs 85\% for global fair allocation). Specifically, the mean utility ratio was much higher for SynData2 vs SynData1 (98\% vs 92\%). Interestingly, there was no statistically significant relationship between the utility ratio and the mean number of population per attribute (Pearson's correlation, $r=-0.85$, $p>0.05$). This can be because of the varying number of attributes that the dataset has.


% \paragraph{FEC}
% \paragraph{UEC}
% \paragraph{WEC}


% \subsubsection{Localized Fair Allocation - SynData2}
% \paragraph{FEC}
% \paragraph{UEC}
% \paragraph{WEC}

\subsubsection{Using Real Data} 
For each year, we implemented each of our 3 models using 3 sets of constraints. Across all the years, the mean ratio of utilities of FEC to \DiRe committees was 0.88 (sd = 0.04), UEC to \DiRe committees was 0.48 (sd = 0.39), and WEC to \DiRe committees was 0.94 (sd = 0.04). As there is only one voter attribute, global fair allocation and localized fair allocation are equivalent. Next, due to Simpson's paradox, we observed that voting on  economic-development-related resolutions that was ``fair'' for all the  continents and all the economic groups of countries was not ``fair'' for economically-underdeveloped countries of Africa.  %Importantly, the algorithmalways terminated in under 102 sec across all instances.



==> FairlyFairMWE - arXiv-4/new_tex/introduction.tex <==

\section{Introduction}
\label{sec:intro}

Fairness is receiving particular attention from the computer science research community. 
%For context, the number of papers that contain the words ``fair'' or ``fairness'' in their titles and are published at top-tier computer science conferences like NeurIPS and AAAI  grew at an average of 38\% year on year since 2018. Moreover, the conference ACM FAccT, formerly known as FAT*, was established in 2018 to ``bring together researchers and practitioners interested in fairness, accountability, and transparency in socio-technical systems''. 
Specifically, there is a growing trend among the Algorithmic Game Theory and the  Computational Social Choice communities toward the use of ``fairness'' \cite{bredereck2018multiwinner,celis2017multiwinner,cheng2019group,flanigan2021fair,hershkowitz2021district,relia2021dire,shrestha2019fairness}. % (not considering Fair Resource Allocation due to the specificity in the use of the word ``fair'').
Moreover, the term is used in varying contexts. For example, Celis \etal \shortcite{celis2017multiwinner} call diversity of candidates in committee elections fairness, Cheng \etal \shortcite{cheng2019group} call representation of voters in committee elections fairness, and Relia \shortcite{relia2021dire} call diversity of candidates \emph{and} representation of voters in committee elections fairness. 
A common denominator across all such papers that guarantee fairness is the use of constraints.
%Such context-specific use of the term narrates an incomplete story of a concept that is far  more complex.
%Merriam-Webster defines ``fairness'' as the quality of being fair or as fair and impartial treatment that lacks favoritism toward one side or another \cite{fairnessDefi}. 
For example, Celis \etal \shortcite{celis2017multiwinner} use diversity constraints to be fair to candidate groups 
%and do not consider fairness from voters' perspective 
and Cheng \etal \shortcite{cheng2019group} use representation constraints to be fair to voter populations. Relia \shortcite{relia2021dire} unified these frameworks to select a diverse and representative (\DiRe) committee.
%do not consider fairness from candidates' perspective. 
%To mitigate such unfairness, \cite{relia2021dire} proposed \emph{\DIRE} Committees, which can guarantee diversity \emph{and} representation in an election. 

% \begin{figure}
%   \centering
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Sample figure caption.}
% \end{figure}



\begin{figure}[t!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.5\textwidth]{new_figures/mainintro_cand_v2.pdf}
  \caption{\textbf{candidates}}
  \label{fig:whatexample/candidates}
\end{subfigure}%
\newline
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\textwidth]{new_figures/mainintro_voters.pdf}
  \caption{\textbf{voters}}
  \label{fig:whatexample/voters}
\end{subfigure}%
\caption{(a) Candidates with ``race'' and ``gender'' attributes (and their Borda scores). (b) Voters with ``state'' attribute. The winning committee (size $k$=4) for California and Illinois, states in the United States, is \{$c_1,c_2,c_3,c_4\}$ and \{$c_5,c_6,c_7,c_8\}$, respectively.}
\label{fig:whatexample}
\end{figure}

\begin{example}
\label{eg-dire}
Consider an election $E$ consisting of $m =8 $ candidates and $n=19$ voters giving ordered preference over $m$ candidates to select a committee of size $k=4$. Each candidate has two attributes, race and gender (Figure~\ref{fig:whatexample/candidates}) (e.g., candidate $c_1$ is a Caucasian male). Voters have one attribute, state (Figure~\ref{fig:whatexample/voters}) (e.g., voters $v_1$ to $v_{10}$ belong to the state of California). The $k$-Borda\footnote{The Borda rule associates score $m - i$ with the $i^{th}$ position, and $k$-Borda selects the candidates with the $k$ highest Borda scores.} winning committee computed for each voter population is  $\{c_1,c_2,c_3,c_4\}$ for California and $\{c_5,c_6,c_7,c_8\}$ for Illinois.
The candidates that form an optimal committee of size $k=4$ consists of $W=\{c_1$, $c_2$, $c_6$, $c_5\}$ with a committee score, $\mathtt{f}(W)=342$. %No other committee can have a score greater than the score of this optimal committee.

\DIRE Committee enforces \emph{diversity constraint} that requires the committee to have at least two candidates of each gender and each race, and a \emph{representation constraint} that requires at least two candidates from the winning committee of each state. Observe that the optimal committee\footnote{For simplicity, the example uses $k$-Borda instead of Chamberlin-Courant rule (discussed in Section~\ref{sec:prelim}). Even when the latter guarantees proportional representation, our motivation of fairly allocating utility holds.}, which is also representative, consists of $W=\{c_1, c_2, c_5, c_6\}$ ($\mathtt{f}(W)=342$), but this committee is not diverse, since all candidates are male. The highest-scoring \DiRe committee is $W'=\{c_1, c_6, c_3, c_8\}$ ($\mathtt{f}(W')=286$).
\end{example}

%The problem of selecting a committee from a given set of candidates arises in multiple domains; it ranges from political sciences (e.g., selecting the parliament of a country) to recommendation systems (e.g., selecting the movies to show on Netflix). Formally, given a set $C$ of $m$ candidates (politicians and movies, respectively), a set $V$ of $n$ voters (citizens and Netflix subscribers, respectively) give their ordered preferences over $C$ to select a committee of size $k$. These preferences can be stated directly in case of parliamentary elections, or they can be derived based on input, such as when Netflix subscribers' viewing behavior is used to derive their preferences.

%A \DiRe committee is a generalized version of the diverse committee \cite{celis2017multiwinner} and the representative committee \cite{cheng2019group,hershkowitz2021district}. 
%Note that a \DiRe committee is a diverse committee when there are no representation constraints and a representative committee when there are no diversity constraints.

%Example~\ref{eg-dire} illustrates the importance of a \DIRE Committee election. 
%considering fairness from the perspective of \emph{all} the actors of an election, namely candidates and voters. 
%However, 
%Yang \etal \cite{yang2019balanced} showed that an unintended consequence of enforcing diversity constraints in ranking is reduced in-group fairness, which refers to the unbalanced loss in utility across groups. Similarly, 
%even though a 
A \DiRe committee ensures fairness in terms of the number of candidates getting selected from candidate groups and voter populations. However, an unintended consequence of enforcing constraints is that it may be fair to various voter populations in a systematically unequal way. Hence, it is important to assess \emph{who} pays \emph{what} cost of fairness. This assessment can be done in multiple ways depending on the context so as to ensure that we fairly allocate fairness across all the voter populations. 

\begin{example}
\label{eg-balanced}
The highest-scoring \DiRe committee selected in Example~\ref{eg-dire} was $W'=\{c_1, c_6, c_3, c_8\}$ ($\mathtt{f}(W')=286$). Note that this outcome fails to select Illinois' highest-ranked candidate ($c_5$), but selects California's highest-ranked candidate ($c_1$). Additionally, if we calculate the total utility derived from the committee by each state, the smaller state achieves lower utility as compared to the larger state (14 versus 16). In contrast, if we select $W''=\{c_1, c_5, c_3, c_8\}$ ($\mathtt{f}(W'')=285$), then both the states get their most preferred candidate and have equal utility (15), at a small cost of the total committee utility.
\end{example}

This example illustrates two techniques\footnote{Similar techniques are well-studied in fair allocation of indivisible goods \cite{freemanrecent}.} that can be used to fairly allocate utility in a \DiRe multiwinner election: (i) selecting the most favorite candidate and (ii) equating utilities received from the winning committee by each population. In either case, without our proposed mitigation techniques, the \DiRe committee is unequally fair across various populations, specifically, harming smaller, historically under-represented populations. % may have to pay a higher cost of fairness (ensuring diversity). 
An important observation we make here is that even if the attributes of the candidates and of the voters \emph{coincide}, we need to treat them separately as fairness to candidates may still cause unfairness to voters. For instance, consider that the voter attribute in Figure~\ref{fig:whatexample/voters} was gender instead of the state. Hence, voters $v_1$ to $v_{10}$ are male and voters $v_{11}$ to $v_{19}$ are female. Therefore, based on Example~\ref{eg-balanced},
%This is because it is different to have, for example, a female candidate elected to the committee than to have a candidate on the committee who is preferred by the female voters, and who themselves may or may not be female.
this change implies that the candidates selected to satisfy the constraints that require a female candidate on the committee systematically led to unequal fairness for female voters, which should not be the case. %the cost of including a female candidate on the committee is borne by female voters more than the male voters, which should not be the case.
%Moreover, a DiRe committee is prone to manipulation by larger voter populations who may strategically vote to ensure smaller populations do not get their most preferred candidate or to ensure that the latter's utility is always lower than the former's. We propose to use methods motivated by the fair division of indivisible goods literature \cite{brandt2016handbook} to circumvent both these  kinds of unfairness. 

%Another unintended consequence of DiRe committee is that it allows manipulation of outcomes. For example, if the California voters in Figure~\ref{fig:whatexample/voters} had a swapped position of $c_5$ and $c_6$, then Illinois' most preferred candidate $c_5$ would have been part of the DiRe committee. However, reordering the preferences among the non-top-$k$ candidates preferred by the Californian voters resulted in an adverse outcome for Illinois, without affecting California. We propose to theoretically check if any of the envyfreeness definitions make the DiRe committee selection problem resistant to manipulation. This is because swapping preferences by Californian voters in the previous example penalizes them as well.



\paragraph{Global, Localized, and Inter-sectional Fair Allocation:} Global fair allocation refers to fair allocation of utility across \emph{all} populations under \emph{all} voter attributes and localized fair allocation refers to fair allocation of utility across \emph{similar} populations under the \emph{same} voter attribute. If there are $\pi$ attributes, then we either do one global fair allocation or $\pi$ localized fair allocation. Localized fair allocation may be needed especially when each voter has more than one attribute. This is because fairly allocating utility between male voters and African-American voters, for example, is not realistic. Fair allocation of utility to male voters should be compared with a voter population under the gender attribute only. On the other hand, inter-sectional fair allocation refers to fair allocation of utility across inter-sectional populations. For example, Caucasian males, Caucasian females, African-American males, and African-American females.

\noindent{\bf Contributions:} 
\begin{itemize}
    \item We develop a model that uses various techniques for fairly allocating candidates across populations in a constrained multiwinner election to mitigate unequal fairness caused among the voter populations.
    \item We propose three variants of the model, namely, global, localized, and inter-sectional.
    \item We study the model theoretically and empirically, and %show that the model makes it hard to manipulate a constrained multiwinner election 
    show the impact of Simpson's paradox between global / localized fair allocation and inter-sectional fair allocation using synthetic and real-world datasets.
\end{itemize}
% In this paper, we define a model that mitigates unfairness to different actors of a system induced by the introduction of fairness.

% The model balances the loss in utility using different metrics. 

% We analyze the model's computational complexity and present an empirical analysis of the balance in utility traded-off across various settings of our model. 
%Overall, our work broadly motivates that a study that uses constraints to guarantee fairness should fairly allocate fairness. A constrained model may systemically be unequally fair to various groups, potentially harming the  historically disadvantaged groups. %assess \emph{who} pays \emph{what} cost to achieve fairness and then fairly allocate fairness.

==> FairlyFairMWE - arXiv-4/new_tex/model+complexity.tex <==
\section{Fairly Allocating Fairness}
\label{sec:Model}

In this section, we formally define a model that maps the \DIRE Committee Winner Determination problem to a problem of fairly allocating indivisible goods. The model mitigates unfairness to the voter population caused by \DIRE Committees. We first define constraints. 

\paragraph{Diversity Constraints,} denoted by $l^D_G \in [1,$ $\min(k, |G|)]$ %\ideally will be better if it is min(k, |G|)
for each candidate group $G \in \mathcal{G}$, enforces at least $l^D_G$ candidates from the group $G$ to be in the committee $W$. Formally,  $\forall$ $G \in \mathcal{G}$, $|G \cap W|\geq l^D_G$. 
%\julia{What's $D$ and why do you need it?  R is also a voting rule.  I wouldn't use D or R; attributes are attributes, if it's for candidates - you call that diversity, if it's for voters - you call that representation.}\kunal{I'll remove it from the attributes. But, we will need it to identify the 2 different types of constraints. I'll change the notation for scoring rule.} \julia{Too late to change now probably, but this is very non-standard notation. What you have here are categorical attributes; each categorical attribute has a cardinality (the number of values); each attribute partitions the candidates or the voters.}
%We note that we do not propose to use the upper bounds as it induces quota system, which is not desirable from social choice perspective. 

%\vspace{-0.15cm}
\paragraph{Representation Constraints,} denoted by $l^R_P \in [1,k]$ for each voter population $P \in \mathcal{P}$, enforces at least $l^R_P$ candidates from the population $P$'s committee $W_P$ to be in the committee $W$. Formally,  $\forall$ $P \in \mathcal{P}$, $|W_P \cap W|\geq l^R_P$.

\begin{definition}
\label{def-DiReCWD}
\textbf{($\mu,\pi$, $\mathtt{f}$)-\DIRE Committee Winner Determination (\DiReCWD):}  We are given an instance of election $E=(C,V)$,  
%set $C$ of $m$ candidates, a set $V$ of $n$ voters such that each voter $v \in V$ has a preference list $\succ_{v}$ over $m$ candidates, 
a committee size $k \in [m]$, a set of candidate groups $\mathcal{G}$ under $\mu$ attributes and their diversity constraints $l^D_G$  $\forall$ $G \in \mathcal{G}$, a set of voter populations $\mathcal{P}$ under $\pi$ attributes and their representation constraints $l^R_P$ and the winning committees $W_P$  $\forall$ $P \in \mathcal{P}$, and a \csr $\mathtt{f}$.
Let $\mathcal{W}$ denote the family of all size-$k$ committees. 
The goal of \DiReCWD is to select committees $W \in \mathcal{W}$ that satisfy  diversity and representation constraints such that $|G\cap W|\geq l^D_G$  $\forall$ $G\in \mathcal{G}$ and $|W_P\cap W|\geq l^R_P$  $\forall$ $P\in \mathcal{P}$ and maximizes, $\forall W \in \mathcal{W}$, $\mathtt{f}(W)$. Committees that satisfy the constraints are \DiRe committees.
\end{definition}


Example~\ref{eg-balanced} showed that a \DiRe committee may create or propagate biases by systematically increasing the selection of lower preferred candidates. This may result in more loss in utility to historically disadvantaged, smaller voter populations.

To mitigate this, we model our problem of selecting a committee as allocating goods (candidates) into $k$ slots. Hence, to assess the quality of candidates being selected from voter populations, we borrow ideas from the literature on the problem of fair resource allocation of indivisible goods \cite{brandt2016handbook}. Formally, given a set of $n$ agents, a set of $m$ resources, and a valuation each agent gives to each resource, the problem of fair allocation is to partition the resources among agents such that the allocation is fair. There are three classic fairness desiderata, namely, proportionality, envy-freeness, and equitability \cite{freemanrecent}. Intuitively, proportionality requires that each agent should receive her ``fair share'' of the utility, envy-freeness requires no agent should wish to swap her allocation with another agent, and equitability requires all agents should have the exact same value for their allocations and no agent should be jealous of what another agent receives. As balancing the loss in utility to candidate groups is analogous to balancing the fairness in ranking \cite{yang2019balanced}, we focus on balancing the loss in utility to voter populations. We propose varying notions of envyfreeness to balance the loss in utility to voter populations\footnote{Our model, \emph{Fairly Allocating} Fairness in Multiwinner Elections, is analogous to a Swiss Army knife. If not as useful as the knife, it can be applicable to more or less any context of a constrained multiwinner election, and the setting of the model can be chosen based on the context.}:


\subsection{Favorite-Envyfree-Committee (FEC)} Each population deserves their top-ranked candidate to be selected in the winning committee. However, selecting a \DiRe committee may result into an imbalance in the candidates selected from each population's ranking. A natural relation of FEC is finding a committee with a bounded level of envy. Specifically, we allow top $x$ ranked in the committee where $x \in [k]$. We call this relaxation FEC up to $x$.
%All proofs are included in the Appendix.

\begin{theorem}\label{thm:FECuptoxP}
Given a \DIRE Committee, there is a polynomial time algorithm that determines whether W', a FEC up to $x$, $\forall x \in \{0,$ $k-2,$ $k-1\}$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{algorithm}[ht!]
\caption{FEC Algorithm}
\label{alg:algorithmFEC}
\begin{flushleft}
\textbf{Input}:\\
$W_P$, $\forall P \in \mathcal{P}$ - winning committee of each population\\
$l_P^R$, $\forall P \in \mathcal{P}$ - diversity constraints\\
$l_G^D$, $\forall G \in \mathcal{G}$ - representation constraints\\
$W$ - Winning \DIRE Committee\\
\textbf{Output}: True if FEC exists, False otherwise\\
\end{flushleft}
%When $x=0$:
\begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=0$}
\STATE $S$ = $\bigcup {c\in C}: \forall P \in \mathcal{P},$ $ \max_{c \in W_P} \mathtt{f}_{\Borda}^{W_P}(c)$

\STATE \textbf{if} $|S|>k$ \textbf{then} \textbf{return} {False}
\STATE \textbf{if} $S\subseteq W$ and  $|S|>0$ \textbf{then} \textbf{return} {True}
\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \cap S|<l_G^D$ \textbf{then} \textbf{return} {False}
\ENDFOR
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $|W_P \cap S|<l_P^R$ \textbf{then} \textbf{return} {False}
\ENDFOR
\STATE \textbf{return} {True}
\ENDIF
% \end{algorithmic}
% %When $x= k-1$:
% \begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=k-1$}
\STATE \textbf{return} {True}
\ENDIF
% \end{algorithmic}
% %When $x=k-2$:
% \begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=k-2$}
\STATE $S$ = $\phi$

\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE $S$ = $W \setminus$ $\{\forall c \in W_P : c$ is the lowest scoring candidate $\mathtt{f}_{\Borda}^{W_P}(c)$ among $W_P\}$
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $|W_P \cap S|<l_P^R$ \textbf{then} \textbf{return} {False}
\ENDFOR

\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \cap S|<l_G^D$ \textbf{then} \textbf{return} {False}
\ENDFOR
\ENDFOR
\STATE \textbf{return} {True}
\ENDIF
\end{algorithmic}
\end{algorithm}


\begin{proof}
Algorithm~\ref{alg:algorithmFEC} clearly runs in time polynomial of the size of input. For correctness, consider the following cases:

\begin{itemize}
    \item \textbf{When $\mathbf{x=0}$}, FEC up to 0 can only exist if $\forall P \in \mathcal{P}$, the population top-scoring candidate $\mathtt{f}_{\Borda}^{W_P}(c)$ is in the committee. Hence, we select each and every top-ranked candidate into set $S$. Then, if set $S$ satisfies all the given constraints, then we know FEC up to 0 exists.
    \item \textbf{When $\mathbf{x=k-1}$}, then existence of a \DiRe committee implies existence of FEC as FEC up to $k-1$ is equivalent to satisfying the requirement that each population has at least one candidate in the committee, which is in line with the definition of the \DiRe committees.
    \item \textbf{When $\mathbf{x=k-2}$}, we iterate over each population $P \in \mathcal{P}$ such that we remove the population's winning committee's $W_P$ least favorite candidate. If the candidates that remain in $W$ satisfy all the constraints after removal of this candidate, then it implies that FEC up to $k-2$ exists. This is because if a \DiRe committee exists even after removing a population's least favorite candidate, then it implies that FEC up to $k-2$ also exists. 
\end{itemize}

\end{proof}

Note that the above theorem encompasses hardness\footnote{The hardness results throughout the paper are under the assumption P $\neq$ NP.} for FEC and FEC up to $x$ as FEC and FEC up to $x$ when $x=0$ are equivalent. 

\begin{theorem}\label{thm:FECuptoxNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a FEC up to $x$, $\forall x \in [1,$ $k-3]$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{proof}
We give a reduction from vertex cover problem on $y$-uniform hypergraphs \cite{garey1979computers} to FEC up to $z$. 

An instance of vertex cover problem on $y$-uniform hypergraphs consists of a set of vertices $X$ = $\{x_1,x_2,\dots,x_{m}\}$ and a set of $|\mathcal{P}|$ hyperedges $S$, each connecting exactly $y$ vertices from $X$. A vertex cover $X' \subseteq X$ is a subset of vertices such that each edge contains at least one vertex from $X$ (i.e. $s\cap X'\neq\phi$ for each edge $s\in S$). The vertex cover problem on $y$-uniform hypergraphs is to find a vertex cover $X'$ of size at most $d$. 

We construct the FEC up to $z$ instance as follows. For each vertex $x \in X$, we have the candidate $c \in C$. For each edge $s \in S$, we have $z+1$ most favorite candidates for each $P \in \mathcal{P}$. Note that we have $|\mathcal{P}|=|S|$. In FEC up to $z$, the requirement is that at least one of the top $z+1$ candidates from each population should be in the committee. Satisfying this requirement ensures that each population is mutually envyfree up to $z$ candidates. Thus, we set $z$ = $y-1$. This corresponds to the requirement that $s\cap X'\neq\phi$. 

Hence, we have a vertex cover $X'$ of size at most $d$  if and only if we have a FEC up to $z$ committee $W$ of size at most $d$ that satisfies the requirement that at least one of the top $z+1$ candidate is in the committee, for all $P \in \mathcal{P}$. 

Note that this reduction holds $\forall z \in [1,$ $k-3]$. 
\end{proof}





\subsection{Utility-Envyfree-Committee (UEC)} Each population deserves to minimize the difference between the utilities each one gets from the selected winning committee, where the utility is the sum of Borda scores that the population gives to the candidates in the winning committee. However, a \DiRe committee may result into an unequal utility amongst all the populations. Formally, for each $P \in \mathcal{P}$, the utility that the population gets from a winning \DiRe committee $W$ is:
    \[ \U_P = \sum_{c \in  W} \mathtt{f}_{\Borda}^{W_P}(c) \]
where $\mathtt{f}_{Borda}^{W_P}(c)$ is the Borda score that candidate $c$ gets based on its rank in population $P$'s winning committee $W_P$. Overall, a UEC is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) = 0 \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| = 0 \]

%\vspace{0.2cm}
\begin{theorem}\label{thm:UECNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a UEC, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{proof}
We give a reduction from the subset sum problem \cite{garey1979computers} to UEC. An instance of subset sum problem consists of a set of non-negative integers $X$ = $\{x_1,x_2,\dots,x_{m}\}$ and a non-negative integer $sum$. The subset sum problem is to determine if there is a subset of the given set with sum equal to given $sum$.  


We construct the UEC instance as follows. We have $|X|$ candidates, which equals to $m$ candidates. Next, we have a $m$-sized scoring vector $\mathbf{s}=\{s_1, s_2, \dots, s_m\}$ such that each $s_i \in \mathbf{s}$ corresponds to $x_i \in X$ sorted in non-increasing order based on the values. Next, we have two population $P$ and $P'$ with $l_P^R= l_{P'}^R$ and let the total utility that population $P$ gets be equal to $sum$. The utility that $P'$ gets from each candidate $c$ depends on the position of $\pos_P(c)$ such that $s_1$ is the utility for candidate on position one, $s_2$ is the utility for candidate on position two, and so on. In UEC, the requirement is that the utility that $P$ gets from a committee $W$ should be the same as the utility $P'$ gets from $W$. Satisfying this requirement ensures that both populations are mutually envyfree. This implies that the total utility that population $P'$ gets from $W$ should be equal to $sum$. This corresponds to the requirement that there is a subset of the given set with sum equal to given $sum$. 

Hence, we have a subset sum if and only if we have a UEC $W$ giving a utility of $sum$ to population $P'$ and $P$.
\end{proof}

A natural relaxation of UEC is UEC up to $\eta$ where $\eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2}]$. This is to say that each population deserves to minimize the difference between utilities from the selected winning committee but up to $\eta$. Hence, a UEC  up to $\eta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|, \eta) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) \leq \eta \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| \leq \eta \]
%\vspace{0.1cm}
\begin{corollary}\label{thm:UECuptoetaNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a UEC up to $\eta$, $\forall \eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2})$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}
    
Note that when $\eta=0$, UEC up to $\eta$ and UEC are equivalent. When $\eta=\frac{(m-1)\cdot(m)}{2}$, UEC up to $\eta$ and \DiRe committee are equivalent.

\begin{proof}
We know that when $\eta=0$, UEC up to $\eta$ and UEC are equivalent. Hence, given that UEC is NP-hard, UEC up to $\eta$ is also NP-hard. Moreover, our reduction in the proof of  Theorem~\ref{thm:UECNP-hard} can be slightly  modified so that it holds $\forall \eta \in \mathbb{Z}: \eta \in \bigl[0,$ $\frac{(m-1)\cdot(m)}{2}\bigr)$. More specifically, we can reduce from subset sum where the sum is within a fixed distance from the given input $sum$ instead of subset sum.

\end{proof}
    
\subsection{Weighted-Envyfree-Committee (WEC)} Each population deserves to minimize the difference between the weighted utilities they get from the selected winning committee. The weighted utility is the sum of Borda scores that the population gives to the candidates in the winning committee who are among their top-$k$ candidates over the maximum Borda score that they can give to candidates based on their representation constraint. Formally, for each $P \in \mathcal{P}$, the weighted utility that the population having representation constraint $l_P^R$ gets from a winning \DiRe committee $W$ is:
    \[ \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \]

Overall, a WEC is a $k$-sized committee such that it aims to

%\[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|) \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| = 0 \]


%\vspace{0.1cm}
\begin{theorem}\label{thm:WECNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a WEC, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{proof}
We give a reduction from the subset sum problem \cite{garey1979computers} to WEC. An instance of subset sum problem consists of a set of non-negative integers $X$ = $\{x_1,x_2,\dots,x_{m}\}$ and a non-negative integer $sum$. The subset sum problem is to determine if there is a subset of the given set with sum equal to given $sum$.  


We construct the WEC instance as follows. We have $|X|$ candidates, which equals to $m$ candidates. Next, we have a $m$-sized scoring vector $\mathbf{s}=\{s_1, s_2, \dots, s_m\}$ such that each $s_i \in \mathbf{s}$ corresponds to $x_i \in X$ sorted in non-increasing order based on the values. Next, we have two population $P$ and $P'$ such that $l_P^R= l_{P'}^R$, $W_P \cap W_{P'} \neq \phi$, and $\{\{W_P \cup W_{P'}\} \setminus \{W_P \cap W_{P'}\}\} \cap W = \phi $. Let the total utility that population $P$ gets be equal to $sum$. Hence, the weighted utility will be 
\[   \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \leq \frac{\sum_{c \in W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{m}m-i} \]

Next, the $sum$ can be written as

\[sum =  \sum_{c \in W} \mathtt{f}_{\Borda}^{W_P}(c)\]

Hence, 
\[    \frac{\sum_{c \in W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{m}m-i} \leq sum  \]

Therefore, \[   \WU_P \leq sum \]



The utility that $P'$ gets from each candidate $c$ depends on the position of $\pos_P(c)$ such that $s_1$ is the utility for candidate on position one, $s_2$ is the utility for candidate on position two, and so on. In WEC, the requirement is that the weighted utility that $P$ gets from a committee $W$ should be the same as the weighted utility $P'$ gets from $W$. Satisfying this requirement ensures that both populations are mutually envyfree. This implies that the total utility that population $P'$ gets from $W$ should be equal to 

\[   \WU_{P'} = \frac{\sum_{c \in W_{P'} \cap W} \mathtt{f}_{\Borda}^{W_{P'}}(c)}{\sum_{i=1}^{l_{P'}^R}m-i} \]

However, as $l_P^R= l_{P'}^R$, we can rewrite $\WU_{P'}$ as 

\[   \WU_{P'} = \frac{\sum_{c \in W_{P'} \cap W} \mathtt{f}_{\Borda}^{W_{P'}}(c)}{\sum_{i=1}^{l_{P}^R}m-i} \]

Additionally, as $W_P \cap W_{P'} \neq \phi$, and $\{\{W_P \cup W_{P'}\} \setminus \{W_P \cap W_{P'}\}\} \cap W = \phi $, we know that the candidates in the winning \DiRe committee is common to both the population. Hence, 

\[\sum_{c \in W_{P'} \cap W} \mathtt{f}_{\Borda}^{W_{P'}}(c) = \sum_{c \in W_{P} \cap W} \mathtt{f}_{\Borda}^{W_{P}}(c)\]

Therefore, we can rewrite $\WU_{P'}$ as

\[   \WU_{P'} = \frac{\sum_{c \in W_{P} \cap W} \mathtt{f}_{\Borda}^{W_{P}}(c)}{\sum_{i=1}^{l_{P}^R}m-i} \]

This implies that 
\[ \WU_{P'} = \WU_{P}\]

However, for this equation to hold, it is necessary that $P'$  gets a total utility of $sum$ from $W$ in line with $P$  getting a total utility of $sum$. This corresponds to the requirement that there is a subset of the given set with sum equal to given $sum$. 

Hence, we have a subset sum if and only if we have a WEC $W$ giving a total utility of $sum$ and weighted utility of $W_P$ to population $P'$ and $P$.
\end{proof}


A natural relaxation of WEC is WEC up to $\zeta$ where $\zeta \in \mathbb{Q}: \zeta \in [0,$ $1]$. This is to say that each population deserves to minimize the difference between weighted utilities from the selected winning committee but up to $\zeta$. Hence, a WEC  up to $\zeta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|, \zeta) \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| \leq \zeta \]

\begin{corollary}\label{thm:WECuptozetaNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a WEC up to $\zeta$, $\forall \zeta \in \mathbb{Q}: \zeta \in [0,$ $1)$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}

Note that when $\zeta=0$, WEC up to $\zeta$ and WEC are equivalent. When $\zeta=1$, WEC up to $\zeta$ and \DiRe committee are equivalent.
\begin{proof}
We know that when $\zeta=0$, WEC up to $\zeta$ and WEC are equivalent. Hence, given that WEC is NP-hard, WEC up to $\zeta$ is also NP-hard. Moreover, our reduction in the proof of  Theorem~\ref{thm:WECNP-hard} can be slightly  modified so that it holds $\forall \zeta \in \mathbb{Q}: \zeta \in [0,$ $1)$. More specifically, we can reduce from subset sum where the sum is within a fixed distance from the given input $sum$ instead of subset sum. $\zeta$ will be a function of this distance and $\forall P \in \mathcal{P}$, $|W_P\cap W|$ and $l_P^R$.

\end{proof}

\subsection{Localized Fair Allocation}

Specifically, we say that an allocation is locally envy-free if no agent envies a neighbor’s allocation and locally proportional if each agent values her own allocation as much as the average value of her neighbor’s allocations, with the former implying the latter. While global envy-freeness implies local envy-freeness, global proportionality does not imply local proportionaity, or vice versa. A general result is that for any two distinct graphs on the same set of nodes and an allocation, there exists a set of valuation functions such that the allocation is locally proportional on one but not the other.




\section{Mitigating Manipulation in \DIRE Elections}

Another unintended consequence and cause of unfairness in \DiRe committees is that it easily allows manipulation\footnote{
All voting mechanisms are known to be susceptible to manipulation \cite{gibbard1973manipulation}, i.e., a situation when a strategizing voter or a group of voters misrepresents his preferences in order to obtain a more desirable outcome. See \cite{elkind2005hybrid} for details.} of outcomes by larger populations to adversely impact smaller, under-represented population. For example, assume Californian voters in Figure~\ref{fig:whatexample/voters} are already manipulated. This is to say that had the California voters \emph{not} swapped position of $c_5$ and $c_6$, then Illinois' most preferred candidate $c_5$ would have been part of the \DiRe committee implicitly. However, the votes are manipulated by changing the preferences among the non-top-$k$ candidates preferred by the Californian voters. This resulted in an adverse outcome for Illinois, without affecting California (see Example~\ref{eg-balanced}).  

\begin{theorem}\label{thm:DiReManipulation-easy}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then there is a polynomial time algorithm that can either help some manipulator population $P \in \mathcal{P}$ manipulate \DiReCWD or determine that \DiReCWD is not manipulable as long as $P$ satisfies the following conditions:
\begin{itemize}
    \item $|P|>|P'|$, $\forall P' \in \mathcal{P}$
    \item $P$ swaps preferences within $C \setminus W_P$
\end{itemize}
\end{theorem}

\begin{algorithm}[ht!]
\caption{\DiReCWD Manipulation Algorithm}
\label{alg:algorithmManipulation}
\begin{flushleft}
\textbf{Input}:\\
$W_P$, $\forall P \in \mathcal{P}$ - winning committee of each population\\
$l_P^R$, $\forall P \in \mathcal{P}$ - diversity constraints\\
$l_G^D$, $\forall G \in \mathcal{G}$ - representation constraints\\
$W$ - Winning \DIRE Committee\\
\textbf{Output}: Manipulated votes if manipulation possible, False otherwise\\
\end{flushleft}

\begin{algorithmic}[1] %[1] enables line numbers
\STATE $P_{\max}$ = $P \in \mathcal{P}:\max(|P|)$
\STATE $E_{\text{actual}}$ = Store the actual votes and $W_P$, $\forall P \in \mathcal{P}$ of election $E$

\FOR{\textbf{each} $c \in C \setminus W_{P_{\max}}$}
\FOR{\textbf{each} $c' \in C \setminus W_{P_{\max}} \setminus c$}
\STATE swap $\pos_v(c)$ and $\pos_v(c')$ for all $v\in P_{\max}$
\STATE $E_{\text{manip}}$ = Store the manipulated votes and corresponding $W_P$,  $\forall P \in \mathcal{P}$ of election $E$
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $W_P \in E_{\text{actual}} \neq W_P \in E_{\text{manip}}$ and $|W_P \in E_{\text{manip}} \cap W\in E_{\text{manip}}|<l_P^R$ \textbf{then} \textbf{return} Maipulated Election $E_{\text{manip}}$
\ENDFOR
\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \in E_{\text{manip}} \cap W\in E_{\text{manip}}|<l_G^D$ \textbf{then} \textbf{return} Maipulated Election $E_{\text{manip}}$
\ENDFOR
\STATE swap $\pos_v(c)$ and $\pos_v(c')$ for all $v\in P_{\max}$
\ENDFOR
\ENDFOR
\STATE \textbf{return} {False}
\end{algorithmic}
\end{algorithm}
\begin{proof}
Algorithm~\ref{alg:algorithmManipulation} clearly runs in time polynomial of the size of input. Note that as $\mathtt{f}$ is a monotone, separable scoring function, we know that 
\[\mathtt{f}(W)=\sum_{c\in W}\mathtt{(c)}\] 
Hence, it implies that computing $W_P$, $\forall P \in \mathcal{P}$ and $W$ for each of the manipulated instance of the election takes polynomial time. For correctness, it is easy to see that the largest population exhaustively swaps each of its bottom $m-k$ candidates and compares the change in outcome. If the outcome changes for any other population or candidate group, then manipulation is successful. Otherwise, the algorithm terminates by returning False.

Note that the algorithm can be easily modified to assess if \emph{any} population can manipulate the election. Instead of choosing the largest population in Line 1 of the algorithm, we can have a For loop that iterates over each population and check whether they can manipulate the result or not.
\end{proof}


For the last theorem, note that the NP-hardness of finding a \DiRe committee does \emph{not} follow and result into NP-hardness of manipulating \DiRe committee elections. This is because we assume that a \DiRe committee is given as an input. In contrast, the next three proofs show that even when \DiRe committees are given, using FEC, UEC, or WEC makes it hard to manipulate \DiRe committee elections. Thus, the models proposed in this paper also mitigate an unintended consequence of imparting fairness (Diversity and Representation constraints) in elections, the consequence being the ease to manipulate elections.


Promisingly, our model has an advantage that even the easiest version of each of the envyfreeness models makes the \DiRe committee selection problem resistant to manipulation. In principle, this is because swapping non-top-$k$ preferences by Californian voters penalizes them as well.


\begin{corollary}\label{thm:DiReManipulationFEC-hard}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a FEC, such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}

\begin{proof}
Theorem~\ref{thm:FECuptoxNP-hard} showed that finding a FEC is NP-hard. Hence, if finding FEC in a regular election is NP-hard, then the hardness of manipulating FEC election follows the hardness of finding a FEC.
\end{proof}
%\vspace{0.1cm}
\begin{corollary}\label{thm:DiReManipulationUEC-hard}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a UEC, such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}
\begin{proof}
Theorem~\ref{thm:UECNP-hard} showed that finding a UEC is NP-hard. Hence, if finding UEC in a regular election is NP-hard, then the hardness of manipulating UEC election follows the hardness of finding a UEC.
\end{proof}
%\vspace{0.1cm}
\begin{corollary}\label{thm:DiReManipulationWEC-hard}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a WEC, such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}

\begin{proof}
Theorem~\ref{thm:WECNP-hard} showed that finding a WEC is NP-hard. Hence, if finding WEC in a regular election is NP-hard, then the hardness of manipulating WEC election follows the hardness of finding a WEC.
\end{proof}

In summary, while mitigating utility-based unfairness caused due to fairness is generally hard, our models make causing manipulation-based unfairness hard as well. The latter intractability is desirable.

%In summary, we deem these proposed notions of envyfreeness among voter populations to be of interest, especially due to the promising empirical results that we got from our initial analysis (discussed in the next section). We also plan to study the theoretical aspects of these notions.

==> FairlyFairMWE - arXiv-4/new_tex/model.tex <==
\section{Fair Allocation Model}
\label{sec:Model}

In this section, we formally define a model that maps the \DIRE Committee Winner Determination problem to a problem of fairly allocating indivisible goods. The model mitigates unfairness to the voter population caused by \DIRE Committees. We first define constraints. 
\vspace{-0.0175cm}
\paragraph{Diversity Constraints,} denoted by $l^D_G \in [1,$ $\min(k, |G|)]$ %\ideally will be better if it is min(k, |G|)
for each candidate group $G \in \mathcal{G}$, enforces at least $l^D_G$ candidates from the group $G$ to be in the committee $W$. Formally,  $\forall$ $G \in \mathcal{G}$, $|G \cap W|\geq l^D_G$. 
%\julia{What's $D$ and why do you need it?  R is also a voting rule.  I wouldn't use D or R; attributes are attributes, if it's for candidates - you call that diversity, if it's for voters - you call that representation.}\kunal{I'll remove it from the attributes. But, we will need it to identify the 2 different types of constraints. I'll change the notation for scoring rule.} \julia{Too late to change now probably, but this is very non-standard notation. What you have here are categorical attributes; each categorical attribute has a cardinality (the number of values); each attribute partitions the candidates or the voters.}
%We note that we do not propose to use the upper bounds as it induces quota system, which is not desirable from social choice perspective. 

\vspace{-0.0175cm}
%\vspace{-0.15cm}
\paragraph{Representation Constraints,} denoted by $l^R_P \in [1,k]$ for each voter population $P \in \mathcal{P}$, enforces at least $l^R_P$ candidates from the population $P$'s committee $W_P$ to be in the committee $W$. Formally,  $\forall$ $P \in \mathcal{P}$, $|W_P \cap W|\geq l^R_P$.

\begin{definition}
\label{def-DiReCWD}
\textbf{\DIRE Committee Winner Determination (\DiReCWD):}  We are given an instance of election $E=(C,V)$,  
%set $C$ of $m$ candidates, a set $V$ of $n$ voters such that each voter $v \in V$ has a preference list $\succ_{v}$ over $m$ candidates, 
a committee size $k \in [m]$, a set of candidate groups $\mathcal{G}$ under $\mu$ attributes and their diversity constraints $l^D_G$  $\forall$ $G \in \mathcal{G}$, a set of voter populations $\mathcal{P}$ under $\pi$ attributes and their representation constraints $l^R_P$ and the winning committees $W_P$  $\forall$ $P \in \mathcal{P}$, and a \csr $\mathtt{f}$.
Let $\mathcal{W}$ denote the family of all size-$k$ committees. 
The goal of \DiReCWD is to select committees $W \in \mathcal{W}$ that satisfy  diversity and representation constraints such that $|G\cap W|\geq l^D_G$  $\forall$ $G\in \mathcal{G}$ and $|W_P\cap W|\geq l^R_P$  $\forall$ $P\in \mathcal{P}$ and maximizes, $\forall W \in \mathcal{W}$, $\mathtt{f}(W)$. Committees that satisfy the constraints are \DiRe committees.
\end{definition}


Example~\ref{eg-balanced} showed that a \DiRe committee may create or propagate biases by systematically increasing the selection of lower preferred candidates. This may result in more loss in utility to historically disadvantaged voter populations.

To mitigate this, we model our problem of selecting a committee as allocating goods (candidates) into $k$ slots. Hence, to assess the quality of candidates being selected from voter populations, we borrow ideas from the literature on the problem of fair resource allocation of indivisible goods \cite{brandt2016handbook}. Formally, given a set of $n$ agents, a set of $m$ resources, and a valuation each agent gives to each resource, the problem of fair allocation is to partition the resources among agents such that the allocation is fair. There are three classic fairness desiderata, namely, proportionality, envy-freeness, and equitability \cite{freemanrecent}. Intuitively, proportionality requires that each agent should receive her ``fair share'' of the utility, envy-freeness requires no agent should wish to swap her allocation with another agent, and equitability requires all agents should have the exact same value for their allocations and no agent should be jealous of what another agent receives. As balancing the loss in utility to candidate groups is analogous to balancing the fairness in ranking \cite{yang2019balanced}, we focus on balancing the loss in utility to voter populations. We propose varying notions of envyfreeness to balance the loss in utility to voter populations\footnote{Our model, \emph{Fairly Allocating} Utility in Constrained Multiwinner Elections, is analogous to a Swiss Army knife. The model is applicable to any context of a constrained multiwinner election and the setting of the model can be chosen based on the context.}:

\begin{table*}[t]
\centering
\begin{tabular}{l|l||c|c||c|c||c|c|c||c|c|c}
\toprule
 & Committee & score & DiRe & \multicolumn{2}{c||}{FEC} & \multicolumn{3}{c||}{UEC} & \multicolumn{3}{c}{WEC}\\
& &  & Committee & \multicolumn{2}{c||}{up to} & \multicolumn{3}{c||}{up to} & \multicolumn{3}{c}{up to}\\
 \cline{5-12}
&  &  &  & 0 & 1 & 0 & 1 & 2 & 0 & $\frac{1}{13}$& $\frac{2}{13}$\\
\midrule
1&$\{c_1, c_2, c_6, c_5\}$&342& \xmark &\cmark&\cmark&\cmark&\cmark&\cmark&\cmark&\cmark&\cmark\\
\hline

2&$\{c_1, c_6, c_3, c_8\}$&286& \cmark &\xmark&\cmark&\xmark&\xmark&\cmark&\xmark&\xmark&\cmark\\
\hline

3&$\{c_1, c_5, c_3, c_8\}$&285& \cmark &\cmark&\cmark&\cmark&\cmark&\cmark&\xmark&\cmark&\cmark\\
\hline

4&$\{c_1, c_5, c_3, c_7\}$&284& \cmark &\cmark&\cmark&\xmark&\xmark&\cmark&\cmark&\cmark&\cmark\\

\bottomrule
\end{tabular}
%}
\caption{Properties satisfied by various example committees selected using the election setup given in Figure~\ref{fig:whatexample/candidates} and Figure~\ref{fig:whatexample/voters}. Each row corresponds to a committee being (row 1) optimal, (row 2) optimal DiRe, (row 3) optimal FEC and optimal UEC given it is DiRe, and (row 4) optimal WEC given it is DiRe. `DiRe' denotes a committee satisfying diversity and representation constraints. `FEC' denotes Favorite-Envyfree-Committee. `UEC' denotes Utility-Envyfree-Committee. `WEC' denotes Weighted-Envyfree-Committee.}

\label{tab:FECUECWEC-examplesummary}
\end{table*}

 \subsection{Favorite-Envyfree-Committee (FEC)} 
 Each population deserves their top-ranked candidate to be selected in the winning committee. However, selecting a \DiRe committee may result into an imbalance in the position of the most-favorite candidate selected from each population's ranking. A natural relaxation of FEC is finding a committee with a bounded level of envy. Specifically, in the relaxation of FEC up to $x$ where $x \in [k]$, rather than selecting the most preferred candidate, we allow for one of the top-$(x+1)$ candidates to be selected. Note that when $x=0$, FEC and FEC up to 0 are equivalent.
%All proofs are included in the Appendix.


Note that the relaxation, FEC up to $x$ is useful when a FEC does not exist. If a FEC exists, then FEC up to $x$ exists for all non-negative $x$. 


 \subsection{Utility-Envyfree-Committee (UEC)} 
%Each population deserves to minimize the difference between the utilities each one gets from the selected winning committee, where the utility is the sum of Borda scores that the population gives to the candidates in the winning committee. However, a \DiRe committee may result in an unequal utility amongst all the populations. Formally, for each $P \in \mathcal{P}$, the utility that the population gets from a winning \DiRe committee $W$ is:
%     \[ \U_P = \sum_{c \in  W} \mathtt{f}_{\Borda}^{W_P}(c) \]
% where $\mathtt{f}_{Borda}^{W_P}(c)$ is the Borda score that candidate $c$ gets based on its rank in population $P$'s winning committee $W_P$. Overall, a UEC is a $k$-sized committee such that it aims to

% % \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|) \]
% % \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) = 0 \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| = 0 \]

% %\vspace{0.2cm}

% A natural relaxation of UEC is UEC up to $\eta$ where $\eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2}]$. This is to say that each population deserves to minimize the difference between utilities from the selected winning committee but up to $\eta$. Hence, a UEC  up to $\eta$ is a $k$-sized committee such that it ensures

% % \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|, \eta) \]
% % \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) \leq \eta \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| \leq \eta \]
% %\vspace{0.1cm}
Each population deserves to minimize the difference between the utilities each one gets from the selected winning committee, where the utility is the sum of Borda scores that the population gives to the candidates in the winning committee. However, a \DiRe committee may result into an unequal utility amongst all the populations. Formally, for each $P \in \mathcal{P}$, the utility that the population gets from a winning \DiRe committee $W$ is:
    \begin{equation} \U_P = \sum_{c \in  W} \mathtt{f}_{\Borda}^{W_P}(c) \end{equation}
where $\mathtt{f}_{Borda}^{W_P}(c)$ is the Borda score that candidate $c$ gets based on its rank in population $P$'s winning committee $W_P$. Overall, a UEC is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) = 0 \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| = 0 \end{equation}

%\vspace{0.2cm}

A natural relaxation of UEC is UEC up to $\eta$ where $\eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2}]$. This is to say that each population deserves to minimize the difference between utilities from the selected winning committee but up to $\eta$. Hence, a UEC  up to $\eta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|, \eta) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) \leq \eta \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| \leq \eta \end{equation}
%\vspace{0.1cm}



Note that in line with FEC, the relaxation, UEC up to $\eta$ is useful when a UEC does not exist. If a committee $W$ is UEC, then it implies that $W$ is UEC up to $\eta$ for all $\eta$ in $[0,$ $\frac{(m-1)\cdot(m)}{2}]$. The relation does not hold the other way, which is to say that if a committee $W$ is UEC up to $\eta$, then it may not be UEC up to $\eta-1$.




% Each population deserves to minimize the difference between the weighted utilities they get from the selected winning committee. The weighted utility is the sum of Borda scores that the population gives to the candidates in the winning committee who are among their top-$k$ candidates over the maximum Borda score that they can give to candidates based on their representation constraint. Formally, for each $P \in \mathcal{P}$, the weighted utility that the population having representation constraint $l_P^R$ gets from a winning \DiRe committee $W$ is:
%     \[ \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \]

% Overall, a WEC is a $k$-sized committee such that it aims to

% %\[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| = 0 \]


% %\vspace{0.1cm}


% A natural relaxation of WEC is WEC up to $\zeta$ where $\zeta \in \mathbb{Q}: \zeta \in [0,$ $1]$. This is to say that each population deserves to minimize the difference between weighted utilities from the selected winning committee but up to $\zeta$. Hence, a WEC  up to $\zeta$ is a $k$-sized committee such that it ensures

% % \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|, \zeta) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| \leq \zeta \]

\subsection{Weighted-Envyfree-Committee (WEC)} Each population deserves to minimize the difference between the weighted utilities they get from the selected winning committee. The weighted utility is the sum of Borda scores that the population gives to the candidates in the winning committee who are among their top-$k$ candidates over the maximum Borda score that they can give to candidates based on their representation constraint. Formally, for each $P \in \mathcal{P}$, the weighted utility that the population having representation constraint $l_P^R$ gets from a winning \DiRe committee $W$ is:
    \begin{equation} \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \end{equation}




Overall, a WEC is a $k$-sized committee such that it aims to

%\[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|) \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| = 0 \end{equation}

\begin{example}
\label{eg-WECcalc}
The highest-scoring \DiRe committee selected in Example~\ref{eg-dire} was $W'=\{c_1, c_6, c_3, c_8\}$ ($\mathtt{f}(W')=286$). The $\WU_{IL}$ will be calculated as follows: Given, $l_{IL}^R$=2, $W_P \cap W = \{c_6, c_8\}$.

\[\WU_{IL} = \frac{\mathtt{f}_{\Borda}^{W_{IL}}(c_6) + \mathtt{f}_{\Borda}^{W_{IL}}(c_8)}{7+6} = \frac{6+4}{7+6}=\frac{10}{13}\]

Similarly, $\WU_{CA}$ will be calculated as follows: Given, $l_{CA}^R$=2, $W_P \cap W = \{c_1, c_3\}$.

\[\WU_{CA} = \frac{\mathtt{f}_{\Borda}^{W_{CA}}(c_1) + \mathtt{f}_{\Borda}^{W_{CA}}(c_3)}{7+6} = \frac{7+5}{7+6}=\frac{12}{13}\]
\end{example}
%\vspace{0.1cm}


A natural relaxation of WEC is WEC up to $\zeta$ where $\zeta \in \mathbb{Q}$ such that $\zeta \in [0,$ $1]$. This is to say that each population deserves to minimize the difference between weighted utilities from the selected winning committee but up to $\zeta$. Hence, a WEC  up to $\zeta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|, \zeta) \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| \leq \zeta \end{equation}


%Observe that the FEC and the UEC committee ($\{c_1, c_5, c_3, c_8\}$) selected in Example~\ref{eg-FEC} and Example~\ref{eg-UEC} is not WEC as $\WU_{IL} = \frac{11}{13}$ and $\WU_{CA}=\frac{12}{13}$.






==> FairlyFairMWE - arXiv-4/new_tex/prelim.tex <==
%\vspace{-.2cm}
\section{Preliminaries and Notation}
\label{sec:prelim}

%\julia{I timed out and didn't get through this section, but I find it confusing that in this section you mix preliminaries, like what's an election, what's $k$-Borda, with defining DiRE committees.  I suggest splitting up into two sections, and changing the flow appropriately.  Preliminaries should really be just preliminaries.  DiRe or DiReCWD should be a separate section.  Also it's important to illustrate all notation, in full sentences. No need for figures, you are ou of space, but a least say, "For example....".}

\paragraph{Multiwinner Elections.} Let $E = (C, V )$ be an election consisting of a candidate set $C = \{c_1,\dots,c_m\}$ and a voter set $V = \{v_1,\dots,v_n\}$, where each voter $v \in V$ has a preference list $\succ_{v}$ over $m$ candidates, ranking all of the candidates from the most to the least desired. $\pos_{v}(c)$ denotes the position of candidate $c \in C$ in the ranking of voter $v \in V$, where the most preferred candidate has position 1 and the least preferred has position $m$. 

Given an election $E = (C,V)$ and a positive integer $k \in [m]$ (for $k \in \mathbb{N}$, $[k] = \{1, \dots, k\}$), a multiwinner election 
%is the one where we 
selects a $k$-sized subset of candidates (or a committee) $W$ using a multiwinner voting rule $\mathtt{f}$ (discussed later) such that the score of the committee $\mathtt{f}(W)$ is the highest. %Formally, given $E = (C,V)$ and $k$, $\mathtt{f}$ outputs the required committee $W$ of exactly $k$ candidates with the highest score. 
We assume ties are broken using a pre-decided priority order.% over all candidates.

%\vspace{-.22cm}
\paragraph{Candidate Groups.} 
%\kunal{For future: The candidates have $\mu$ attributes, $A_1 , . . . , A_\mu$. Each attribute $A_i$, for all $i \in [\mu]$, partitions the candidate into $g_i$ groups, $\group{i}{1} , . . . , \groupsub{i}{g} \subseteq C$. The set $\mathcal{G}$ of \emph{all} such groups will be $\group{1}{1} , . . . , \groupsub{\mu}{g} \subseteq C$.}
The candidates have $\mu$ attributes, $A_1 , . . . , A_\mu$, such that $\mu \in \mathbb{Z}$ and $\mu \geq 0$. Each attribute $A_i$, $\forall$ $i \in [\mu]$, partitions the candidates into $g_i \in [m]$ groups, $\group{i}{1} , . . . , \groupsub{i}{g} \subseteq C$. Formally, $\group{i}{j} \cap  \group{i}{j'} = \emptyset$, $\forall j,j' \in [g_i], j \ne j'$. For example, candidates in Figure~\ref{fig:whatexample/candidates} have race and gender attribute  ($\mu$ = 2) with disjoint groups per attribute, male and female ($g_1$ = 2) and Caucasian and African-American ($g_2$ = 2). Overall, the set $\mathcal{G}$ of \emph{all} such arbitrary and potentially non-disjoint groups is $\group{1}{1} , . . . , \groupsub{\mu}{g} \subseteq C$. %Note that the number of groups a candidate belongs to is equal to the number of attributes $\mu$. 

%Candidates are divided into a set $\mathcal{G}$ of arbitrary and potentially non-disjoint 
%groups $\group{1}{1} , . . . , \groupsub{\mu}{g} \subseteq C$ over $A_1 , . . . , A_\mu$  
%$A_1^D , . . . , A_\mu^D$ 
%candidate attributes. Each attribute $A_i$, for all $i \in [\mu]$, has $g_i$ groups. Groups under each attribute $A_i$, for all $i \in [\mu]$, are disjoint. Formally, $\group{i}{j} \cap  \group{i}{j'} = \emptyset$, $\forall j,j' \in [g_i]$. For example, candidates in Figure~\ref{fig:example/candidates} have one attribute gender ($\mu$ = 1) with two groups, male and female ($g_1$ = 2). %Here, the number of candidate attributes $\mu=1$ and the number of groups $g_1$=2.
%(e.g., if we only have one attribute race, which has two groups Caucasian and African-American, then the number of candidate attributes $\mu=1$ and the corresponding number of groups $g_1$=2).
%\julia{Explain notation in full sentences, here and elsewhere, not in (e.g.,\dots) in parentheses.  For example, \dots.} 

%We note that we do not propose to use the upper bounds as it induces quota system, which is not desirable from social choice perspective. % \kunal{Julia, can you please help me with citation that shows quota is bad?}.  \julia{No need to substantiate with a citation.  This is not a scientific fact, it's just not a thing we accept in our society today.}
%\vspace{-.22cm}

\paragraph{Voter Populations.}
The voters have $\pi$ attributes, $A'_1 , . . . , A'_\pi$, such that $\pi \in \mathbb{Z}$ and $\pi \geq 0$. The voter attributes may be different from the candidate attributes. Each attribute $A'_i$, $\forall$ $i \in [\pi]$, partitions the voters into $p_i \in [n]$ populations, $\population{i}{1} , . . . , \populationsub{i}{p} \subseteq V$. Formally, $\population{i}{j} \cap  \population{i}{j'} = \emptyset$, $\forall j,j' \in [p_i], j \ne j'$. For example, voters in Figure~\ref{fig:whatexample/voters} have state attribute  ($\pi$ = 1), which has populations California and Illinois ($p_1$ = 2). Overall, the set $\mathcal{P}$ of \emph{all} such predefined and potentially non-disjoint populations will be $\population{1}{1} , . . . , \populationsub{\pi}{p} \subseteq V$. 

%The number of populations a voter belongs to is equal to the number of attributes $\pi$. 
Additionally, we are given $W_P$, the winning committee $\forall$ $P \in \mathcal{P}$. We limit the scope of $W_P$ to be a committee instead of a ranking of $k$ candidates because when a \csr such as CC rule is used to determine each population’s winning committee $W_P$, then a complete ranking of each population’s collective preferences is not possible. 
%We note that a fine-grained accounting of representation is not possible in our model. This is because when a \csr such as Chamberlin-Courant rule is used to determine each population’s winning committee $W_P$, then a complete-ranking of each population’s collective preferences is not possible. Thus, we have design our model to only consider each population's winning committee $W_P$.

%The voters are divided into a set $\mathcal{P}$ of populations $\population{1}{1} , . . . , \populationsub{\pi}{p} \subseteq V$ over $A'_1 , . . . , A'_\pi$ voter attributes, which may be different from candidate attributes. Each attribute $A'_i$, for all $i \in [\pi]$, has $p_i$ populations. Populations under each attribute $A'_i$, for all $i \in [\pi]$, are disjoint. Formally, $\population{i}{j} \cap  \population{i}{j'} = \emptyset$, $\forall j,j' \in [p_i]$. For example, voters in Figure~\ref{fig:example/voters} have one attribute state ($\pi$ = 1), which has two populations California and Illinois ($p_1$ = 2). 
%Here, the number of voter attributes $\pi=1$ and the  number of populations $p_1$=2.
%We are given $W_P$, the winning committee of each population $P \in \mathcal{P}$.

\paragraph{Multiwinner Voting Rules.} There are multiple types of multiwinner voting rules, also called committee selection rules. 
%as we now call them. 
%For example, a Condorcet principle based selection rule selects a committee that is at least as strong as every other committee in a pairwise majority comparison \cite{darmann2013hard,faliszewski2016committee}, and in an approval-based selection rule, each voter submits an \emph{approval ballot} approving a subset of at least $k$ candidates; the \emph{ballot profile} consisting of all voters' \emph{approval ballots} is then used to select a committee \cite{faliszewski2016committee,kilgour2010approval,sanchez2017proportional}. 
In this paper, we focus on committee selection rules $\mathtt{f}$ that are based on single-winner positional voting rules, and are
%. These committee selection rules are 
monotone and submodular ($\forall A \subseteq B, f(A) \leq f(B)$ and $f(B) \leq f(A) + f(B \setminus  A)$).% \cite{bredereck2018multiwinner,celis2017multiwinner}. %($f : 2^{[m]} \rightarrow R_{\geq0}$ such that $f(A\cup B)+f(A\cap B)\leq f(A)+f(B)$, for all $A,B \subseteq [m]$). 

% \begin{definition}
% \label{def-monroe} \kunal{remove this. not used.} The Monroe rule \cite{monroe1995fully} divides the $n$ voters into $k$ populations (assuming $k$ divides $n$).
% Then, each population's most preferred candidate is selected into the $k$-sized committee. Formally, for each population, say $P$, select the candidate $c$ that has the highest score for that population: $MAX_{c \in C}(score_{P}(c))$.
% \end{definition}

%\vspace{-.075cm}
\begin{definition}
\label{def-CC} \textbf{Chamberlin–Courant (CC) rule \cite{chamberlin1983representative}:}
%Chamberlin–Courant (CC) rule 
The CC rule  associates each voter with a candidate in the committee who is their most preferred candidate in that committee. 
 %For each possible $k$-sized committee $W \in \mathcal{W}$, calculate the score each voter gives to their most preferred candidate $c$ $\in$ $W$. 
 The score of a committee is the sum of scores given by voters to their associated candidate. 
 Specifically, $\mathbf{\beta}$-CC uses the Borda positional voting rule such that it assigns a score of $m-i$ to the $i^{\text{th}}$ ranked candidate who is their highest-ranked candidate in the committee.

    %  \begin{itemize}
    %     % \item $\mathbf{\alpha -CC}$ uses $k$-approval positional voting rule such that it assigns a score of 1 if the highest ranked candidate in the committee is among the top $k$ candidates in their preferences, 0 otherwise.
        
    %     \item $\mathbf{\beta -CC}$ uses Borda positional voting rule such that it assigns a score of $m-i$ to the $i^{th}$ ranked candidate who is their highest ranked candidate in the committee.
    % \end{itemize}
\end{definition}
%\vspace{-.1cm}
% \begin{definition}
% \label{def-monroe} \textbf{Monroe rule:} The Monroe rule \cite{monroe1995fully} dynamically divides the $n$ voters into $\pi$ populations based on the cohesiveness of their preferences %\julia{how does it divide them, just randomly assigning each voter to their respective population?  doesn't make sense, you'll get different committees depending on how you happen to divide....  or is the mapping of voters to populations given as input? \kunal{Yes, in our case, mapping of voters to populations given as input.}} 
% where $\pi$ = $k$ (assuming $k$ divides $n$).
% %\julia{why do we assume this, are these populations of equal size? \kunal{generally, this condition is needed when predefined voter subpopulations are not given, but in our case specifically, this won't be needed.}}). 
% Then, each subpopulation's most preferred candidate is selected into the $k$-sized committee. Formally, $\forall$ $P \in \mathcal{P}$, select $c$ for $P$ : $\max_{c \in C}(\mathtt{f}_{P}(c))$. %In other words, each candidate in the committee is represented by an equal number of voters.
% \end{definition}
%\vspace{-.05cm}
A special case of submodular functions are separable functions: %, which calculate the score of committee as follows: 
score of a committee $W$ is the sum of the scores of individual candidates in the committee. Formally, $\mathtt{f}$ is separable if it is submodular and $\mathtt{f}(W) = \sum_{c \in W}^{}\mathtt{f}(c)$ \cite{bredereck2018multiwinner}. %We define the following 
Monotone and separable selection rules are natural and are considered good when the goal of an election is to shortlist a set of individually excellent candidates:

% \begin{definition}
% \label{def-sntv} \textbf{Single non-transferable vote (SNTV) rule:}
% %The SNTV rule 
% outputs committee of $k$ candidates with the highest plurality scores.
% %outputs committee of top-$k$ plurality scoring candidates.
% \end{definition}


\begin{definition}
\label{def-kborda} \textbf{$k$-Borda rule} The $k$-Borda rule
%$k$-Borda rule 
outputs committees of $k$ candidates with the highest Borda scores.
%outputs committee of top-$k$ Borda scoring candidates.
\end{definition} 


%As discussed in Section~\ref{sec:intro}, the use of the term fairness in computer science research is increasing. For context, the number of papers that contain the words ``fair'' or ``fairness'' in their titles and are published at top-tier computer science conferences like AAAI and NeurIPS  grew at an average of 38\% year on year since 2018. Similarly, fairness in multiwinner election also received particular attention. To this end, a series of papers \cite{bredereck2018multiwinner,celis2017multiwinner,relia2021dire} discussed various aspects of fairness. Building upon these papers and as a generalizable work that impacts all fairness researchers, we discuss the importance to assess \emph{who} pays \emph{what} cost of fairness. 
Note that we focus on fairly allocating candidates \emph{only} across voter populations. This is because monotone, submodular scoring functions like $\beta$-Chamberlin Courant do not give scores to individual candidates. Hence, there is no way to fairly allocate candidates across candidates groups as these rules score a committee and not each candidate. We used $k$-Borda in Examples ~\ref{eg-dire} and \ref{eg-balanced} for simplicity.


%All scoring functions are assumed to be submodular unless specifically mentioned to be separable.


%\kunal{remove this.} Multiwinner elections that have predefined voter subpopulations are carried out in a sequence of steps, depicted in Figure~\ref{fig:election}. While specifics of the steps differ between different election schemes, the overall structure remains the same. Specifically, we have candidates belonging to multiple non-disjoint attribute groups (Figure~\ref{fig:election}(a)) and we have voters, partitioned into disjoint subpopulations.  As the first step, ``\pe'', voter preferences are collected in the form of candidate rankings (Figure~\ref{fig:election}(b)). Next, during the ``\va'' step, (i) scores are assigned to each candidate for each voter using some voting rule, and (ii) per-candidate scores are aggregated across voters to compute the subpopulation consensus ranking (Figure~\ref{fig:election}(c)). Finally, the ``\cs'' step chooses candidates from subpopulation consensus rankings using \emph{committee selection rules}\footnote{These rules are typically referred to as ``multiwinner voting rules'' in the literature, but we refer to them as ``committee selection rules'' to   explicitly distinguish between the steps in the election process.}, which may further assign scores to candidates and aggregate these, or use the ranked lists directly.

% %\section{Single-winner positional scoring rules}
% \section{Single-winner Voting Rules}
% \label{sec:prelim/singlerules}

% A single-winner scoring function $\gamma_m : [m] \rightarrow \mathbb{R}_+$ associates each possible position in a vote with a score. (We omit $m$ and write simply  $\gamma$ when $m$ is clear from context.) For example, plurality scoring function associates score 1 with the top position and score 0 with all the other positions, $k$-approval scoring function associates score 1 with the top $k$ ranked candidates and score 0 with all the other positions, and the Borda scoring function associates score $m - i$ with the $i^{th}$ position. 

% %\julia{Call this step aggregation of whatever terminology you decide to use, see my comment in 2.1.\kunal{changed.}} 
% The total score of a candidate $c$ in an election $E = (C,V)$ is thus defined as $score(c) = \sum_{v\epsilon V}^{} \gamma(pos_v(c))$. We use this setup for the \va step shown in Figure~\ref{fig:election}. Specifically, for each voter within a subpopulation, we use one of the above discussed voting rules to assign scores to candidates based on the position they take in the voter's preferences, and then aggregate these scores to compute subpopulation consensus ranking. In the event of two (or more) candidates getting the same aggregated score, the tied candidates are ranked as if they were the highest member of the tie, and hence, they occupy the same, higher position in the consensus ranking \cite{kendall1945treatment}. The candidate ranked after them continues to occupy the position she would have occupied had there not been a tie.
% %The discussion in this section is focused on single-winner positional voting rules, in line with our focus on multiwinner voting rules for ordered preferences in the next section.
% %, in line, with our focus on OWA (ordered weighted average) or committee positional scoring rule for multiwinner election in the next section.
% %\julia{this is specifically about positional scoring rules, make that clear, briefly state what other kinds there are. \kunal{we have discussed the types of multiwinner voting rules, and as this document is about multi-winner voting, stating other kinds of single-winner voting rules may not be a good idea. Particularly, I didn't see any paper discuss single-winner voting rules beyond what was required for the document.}}


% %SNTV, Bloc, and k-Borda, are polynomial- time computable: It suffices to output a committee consisting of k candidates with the highest Plurality, k-Approval, or Borda scores, respectively. The Chamberlin–Courant rule and the Pessimist rule are NP-hard (formally, the problem of deciding if there is a committee with at least a given score is NP-complete for these rules; see the works of Procaccia et al. [2008] and Lu and Boutilier [2011] for the case of the Chamberlin–Courant rule, and the work of Skowron et al. [2016] for the Pessimist rule)

% %nsequently, to a variety of different algorithmic problems. Prevalent ex- amples include committee scoring rules [Aziz et al., 2017b; Elkind et al., 2014], approval-based rules [Aziz et al., 2017a], OWA-based rules [Skowron et al., 2015b], variants of the Monroe rule [Betzler et al., 2013; Monroe, 1995; Skowron et al., 2015a] and the goalbase rules [Uckelman et al., 2009].











% \section{Multiwinner Voting Rules (Committee Selection Rules)}
% \label{sec:prelim/multirules}
% We recall that there are multiple types of multiwinner voting rules, or committee selection rules as we now call them. %\julia{Don't call these ``voting rules'', call them committee selection rules or something similar, to disambiguate.  Adjust terminology in the rest of this section accordingly. \kunal{changed throughout the document.}} 
% For example, a Condorcet principle based selection rule selects a committee that is at least as strong as every other committee in a pairwise majority comparison \cite{darmann2013hard, faliszewski2016committee}, and in an approval-based selection rule, each voter submits an \emph{approval ballot} approving a subset of at least $k$ candidates; the \emph{ballot profile} consisting of all voters' \emph{approval ballots} is then used to select a committee \cite{faliszewski2016committee, kilgour2010approval, sanchez2017proportional}. 

% In this document, we focus on committee selection rules that are based on single-winner positional voting rules to select a committee based on subpopulation's consensus ranking in the \cs step depicted in Figure~\ref{fig:election}.  These rules are very common and suffice to express many natural problems where ordered preferences are given \cite{bredereck2018multiwinner}.  These rules are also interesting from the computational perspective because some select a committee in polynomial time, while others are provably hard \cite{celis2017multiwinner}. Specifically, we use selection rules that are monotone and submodular. 

% \textbf{Monotone:} A function is said to be monotone if adding an element to a set does not decrease its value. Formally, $\forall A \subseteq B$, $f(A) \leq f(B)$. In other words, the empty set has the lowest possible value, 0, and the set containing all elements has the highest possible value.
% \begin{example}
% \label{eg-monotone} {}
% Consider scores of candidates from Figure~\ref{fig:election}(d1). A committee of size 2 containing $c_1$ and $c_2$ (set $A$) has score of 14,300. Adding any candidate to this set $A$ will never decrease its score.
% \end{example}


% \subsection{Submodular Selection Rules}
% %\julia{I finally understand what's confusing.  There are two steps here, each done by a different kind of a rule.  The first step is when each voter assigns a score to each candidate.  Scoring rules like plurality and Borda govern that.  And then there is another set of rules that we use to decide how to combine (aggregate) the scores of the candidates across the voters.  For example, for Monroe, Definition 1 tells us how to pick candidates from each subpopulation into a committee, but it doesn't tell us how subpopulation preferences are derived.  Can you use, \eg, Borda for step 1, aggregate candidate scores in each subpopulation by summing them, and then use Monroe for step 2?  In Figure 1.1, you denote one of these transitions as "aggregate preferences" and the other as "calculate candidate scores using Borda voting rule", but, really, it's not always Borda for going from (c) do (d).  If I understand this correctly now --- it's very important to make this distinction, and to use different terms to denote the operations in each step.  Also, when you give examples, you need to show not only the result, but also how that result is computed step-by-step. \kunal{updated example 1 to clarify this. Shared more details in the reply to your email.}}

% %\julia{This section still needs work.}
% Submodular functions capture the notion of diminishing returns with increasing input size. More precisely, a submodular function has the property that, as the size of the input set increases, the difference in the incremental value of the function made by adding a single element decreases. Formally, a function $f$ is said to be submodular if $f$ satisfies the following: $\forall A \subseteq B$, if $f(A) \leq f(B)$ ($f$ is monotone), then 
% %$f(A\cup B) + f(A\cap B) \leq f(A) + f(B)$
% $f(B) \leq f(A) + f(B \setminus  A)$
% \cite{celis2017multiwinner,schrijver2003combinatorial}. We usually select committee selection rules to be submodular. 
% %\julia{what happens if $f$ is not monotone? \kunal{(1) In our context, if $f$ is not monotone, it means that adding a candidate to the committee may decrease the committee's score, which doesn't make sense.}}
% We define the following monotone and submodular committee selection rules:
% \begin{definition}
% \label{def-monroe} {\rm[Monroe rule]:} The Monroe rule \cite{monroe1995fully} divides the $n$ voters into $\pi$ subpopulations %\julia{how does it divide them, just randomly assigning each voter to their respective population?  doesn't make sense, you'll get different committees depending on how you happen to divide....  or is the mapping of voters to populations given as input? \kunal{Yes, in our case, mapping of voters to populations given as input.}} 
% where $\pi$ = $k$ (assuming $k$ divides $n$).
% %\julia{why do we assume this, are these populations of equal size? \kunal{generally, this condition is needed when predefined voter subpopulations are not given, but in our case specifically, this won't be needed.}}). 
% Then, each subpopulation's most preferred candidate is selected into the $k$-sized committee. Formally, for each subpopulation, say $P_i$, select the candidate $c$  that has the highest score for that subpopulation: $MAX_{c \in C}(score_{P_{i}}(c))$. %\julia{I feel like I asked this many times --- what if some populations agree on their favorite candidate?  How is the next candidate chosen to get a committee of size $k$, arbitrarily among the second most preferred candidates? \kunal{Julia, in this section, there is already a lot of information being given to the readers. Hence, we may want to keep it simple and stick to the textbook definitions here. To this end, I have already addressed this issue as the first thing in the next section in detail. Please see Example~\ref{eg2-opt} and the paragraph after that.}}
% \end{definition}

% \begin{example}
% \label{eg-Monroe} {}
% Consider the voters and their preferences in Figure~\ref{fig:election}(b). If we were to select a committee of size, say $k$=3, then we divide voters into 3 subpopulations based on the state the voter belongs to (Figure~\ref{fig:election}(c)), and each subpopulation's most preferred candidate, determined using plurality, is selected into the committee. Hence, $c_1$, $c_5$, and $c_6$ will be selected into the committee. %\julia{not clear how we divide voters into subpopulations, and who the winning candidates would be in this example. \kunal{Changed the example. Also, highlighted how Monroe is same as CC as this rule can be used when $\pi$ = $k$. In retrospect, we can remove this rule from the discussion if needed.}}
% \end{example}

% \begin{definition}
% \label{def-CC} {\rm[Chamberlin–Courant (CC) rule]:} 
% %\julia{This is still not clear, it reads like --- the committee exists and we are assigning already selected candidates to populations, but it's the other way around.  First we compute the consensus for each subpopulation.  Then we select each subpopulation's most preferred candidate and add it to the committee.  The score of the committee is the sum of scores of the candidates, the only question is --- are the scores really taken just from the population that nominates the candidate?  doesn't make a ton of sense, since each population votes for each candidate in any case.  Once you define better terminology and notation in Section 2.1, you can easily use it here. \kunal{I think neither of this is what is happening. Also, score of the committee is \textbf{not} sum of scores of the candidates. This would specifically be a separable function had this been the case. Also, a subpopulation just has one representative in the committee, and the representative is their highest scoring candidate present in the committee. I am sure that based on definitions of CC in \cite{bredereck2018multiwinner, celis2017multiwinner, diss2018chamberlin}, this is what happens technically: Say a committee exists. In our case, each subpopulation assigns a score to the committee based on the score they would assign to their highest preferred candidate present in the committee. We do this for all possible committees, and select a committee who gets the highest score. But in practice, we can always do what you suggested: select each subpopulation's most preferred candidate, compute its score taken just from the subpopulation that nominates the candidate, and add it to the committee (if $k$ $\geq$ $\pi$), and add any candidate to the committee there after (see Example~\ref{eg2-opt} for details.) But, I think in this section, we should stick to the textbook definition of CC, and discuss any limitations it may possess in the next section, like we do currently.}}
% Chamberlin–Courant (CC) rule \cite{chamberlin1983representative} associates each voter subpopulation with a candidate in the committee who is their most preferred candidate in that committee. The score that a subpopulation gives to this most preferred candidate from the committee is the score they give to the committee. In our context, for each possible committee $\mathtt{R}(E,k)$ of size $k$, we calculate the score each voter subpopulation gives to their most preferred candidate $c$ in $\mathtt{R}(E,k)$. The score of the committee is the sum of scores given by voter subpopulations that rank candidate $c$ the highest.
 
%  %has a positional scoring function $\gamma(pos_v(c))$ : $\forall 1\leq i,j \leq m$, if $ 1 \leq pos_v(c_i) \leq pos_v(c_j)\leq m$ then $\gamma(pos_v(c_i)) \geq \gamma(pos_v(c_j))$. 
% % \julia{the ``if'' part is invalid. also, you are saying somthing about all valid pairs of indexes $i$ and $j$, but we never assumed that an ordering of candidates is given apriori.  What does this rule say in words? If a candidate is ranked higher than another, then its score is no lower than that of the other?  Something like this? Also, notation is only useful if it helps us understand things, or if it's used later.  I don't see $\gamma$ being used later.}
%  %\kunal{In words: each voter's score to the committee is the score she assigns to her most preferred committee member. In our context, for each possible committee $\mathtt{R}(E,k)$ of size $k$, we calculate the score each voter subpopulation gives to their most preferred candidate $c$ in $\mathtt{R}(E,k)$. The score of the committee is the sum of scores given by voter subpopulations that rank candidate $c$ the highest. I agree, we don't use notation for CC voting rule anywhere else. We can describe it in words.}
%  %\julia{No, I asked about the notation above, not below.  The notation that describes the positional scoring function.  What's the significance of saying that i and j are between 1 and m?   You need to go over definition 2 in its entirety and write it down with just the right amount of notation to make it precise.  The current notation is convoluted, and at least some of it is unnecessary.  Above, I don't think you need $\gamma$, you can use $score$.} 
%      \begin{itemize}
%         \item $\mathbf{\alpha -CC}$ is a \csr that uses $k$-approval positional voting rule such that it assigns a score of 1 if the highest ranked candidate in the committee is among the top $k$ candidates in their preferences, 0 otherwise.
%         %$\forall pos_v(c) \leq k$, $\gamma(pos_v(c))$ $= 1$, and $\gamma(pos_v(c)) = 0$ otherwise. 
%         \item $\mathbf{\beta -CC}$ is a \csr that uses Borda positional voting rule such that it assigns a score of $m-i$ to the $i^{th}$ ranked candidate who is their highest ranked candidate in the committee.
%         %$\mathbf{\beta -CC}$ uses a positional scoring function such that $\forall pos_v(c) \leq m$, $\gamma(pos_v(c))$ $= m - pos_v(c)$. 
%     \end{itemize}
% \end{definition}

% \begin{example}
% \label{eg-a-CC} {}
% Consider the consensus preferences in Figure~\ref{fig:election}(c). If we were to select a committee of size, say $k$=3, using $\mathbf{\alpha -CC}$, then for each voter subpopulation, the selection rule will give a score of 1 to candidate $c$ if $c$ is among the top $k$ candidates for that subpopulation. For example, candidate $c_1$, $c_2$ and $c_4$ are among top 3 for California, so they will score 1x1000 (size of subpopulation) to any committee that has at least one of these 3 candidates. Similarly, Oklahoma and Oregon will give a score of 1x100 each to the committee if one their top 3 candidates is in the committee. Committee consisting of candidates $c_1$, $c_7$, and $c_6$ is one of the multiple highest scoring committees that can be selected using this rule. 
% \end{example}

% \begin{example}
% \label{eg-b-CC} {}
% Consider the consensus preferences in Figure~\ref{fig:election}(c). If we were to select a committee of size, say $k$=3, using $\mathbf{\beta -CC}$, then for each voter subpopulation, the selection rule will give a score of $m-i$ to the highest ranking candidate $c$ who is on $i^{th}$ position. For example, candidate $c_1$ is at the 1$^{st}$ position for California which results in score of 7 ($m-i$ = 8 - 1) x 1000 (size of California) = 7000 by California to the committee. Similarly, Oklahoma and Oregon also give a score to the committee based on their top scoring candidate. Hence, a committee selected using this rule will consist of $c_1$, $c_5$, and $c_6$, each one being the most preferred candidate of a subpopulation, and having a score of 8,400 (7x1000 (California) + 7x100 (Oklahoma) + 7x100 (Oregon)).
% \end{example}

% \subsection{Separable Selection Rules}
% A special case of submodular functions are separable functions\footnote{Henceforth, we refer to submodular functions that are separable as ``separable functions'', and to submodular functions that are \emph{not} separable as simply ``submodular functions''.}. 
% Separable functions calculate the score of committee as follows: Score of a committee $\mathtt{R}(E,k)$ is the sum of the scores of individual candidates in the committee. Formally, $score(\mathtt{R}(E,k)) = \sum_{c \in \mathtt{R}(E,k)}^{}score(c)$ \cite{bredereck2018multiwinner}.
% We define the following monotone and separable selection rules:

% \begin{definition}
% \label{def-sntv} {\rm[single non-transferable vote rule]:}
% {Single non-transferable vote rule} (the SNTV rule) outputs committee of $k$ candidates with the highest plurality scores.
% \end{definition}


% \begin{definition}
% \label{def-kborda} {\rm[$k$-Borda rule]:}
% $k$-Borda rule outputs committee of $k$ candidates with the highest Borda scores.
% \end{definition} 

% \begin{example}
% \label{eg-kBorda} {}
% Consider the Borda scores of candidate preferences in Figure~\ref{fig:election}(d1). A committee selected using $k$-Borda will consist of top $k$ scoring candidates where score of each candidate is determined using Borda voting rule. Hence, a committee of size 4 (=$k$) will consist of $c_1$, $c_2$, $c_4$, and $c_3$ (Figure~\ref{fig:election}(d2)), and a committee of size 3 (=$k$) will consist of $c_1$, $c_2$, and $c_4$. It should be noted that this committee, selected using $k$-Borda ($k$=3) is different from the the committee selected using $\beta$-CC (Example~\ref{eg-b-CC}).
% \end{example}

==> FairlyFairMWE - arXiv-4/new_tex/related_work.tex <==
%\vspace{-.2cm}
\section{Related Work}
\label{sec:RW}


%Our work is at an intersection of multiple ideas, and hence, in this section, we briefly summarize the related work spread across different domains, some of which we already discussed in the previous section.

Our work primarily builds upon the literature on constrained multiwinner elections. Goalbase score functions, which specify an arbitrary set of logic constraints and let the score capture the number of constraints satisfied, could be used to ensure diversity \cite{uckelman2009representing}. Using diversity constraints over multiple attributes in single-winner elections is NP-hard \cite{lang2018multi}. Also, using diversity constraints over multiple attributes in multiwinner elections and participatory budgeting is NP-hard, which has led to approximation algorithms and matching hardness of approximation results by Bredereck \etal \shortcite{bredereck2018multiwinner} and Celis \etal \shortcite{celis2017multiwinner}. Finally, due to the hardness of using diversity constraints over multiple attributes in approval-based multiwinner elections \cite{brams1990constrained}, these have been formalized as integer linear programs (ILP) \cite{potthoff1990use}. In contrast, Skowron \etal \shortcite{skowron2015achieving} showed that ILP-based algorithms fail in the real world when using ranked voting-related unconstrained proportional representation rules. 
%like Chamberlin-Courant and Monroe rules, even when there are no constraints.



%Overall, we discussed previous work on hardness of unconstrained and constrained multiwinner elections, and the use of techniques like ILP and approximation algorithms in this field. 


%In summary, our work differs as we: (i) consider elections with predefined voter populations, (ii) delineate voter and candidate attributes, and (iii) consider representation \emph{and} diversity constraints. No previous work, to the best of our knowledge, has considered fairness from the perspective of voter attributes.

% \cite{shrestha2019fairness}.%, (iii) they assume that number of voter subpopulations will be greater than or equal to committee size, and (iv) they provide the flexibility to upper bound the number of candidates selected from each group which may essentially be analogous with the quota system.


%\kunal{Lang and Skowron (2016) considered a model of diversity requirements that closely resembles our interval constraints. There are two main differences between their work and ours: (i) they do not consider objective functions and (ii) their input consists of “ideal points” instead of intervals for each label; since there might not exist a committee satisfying such “exact” constraints, they focus on finding committees minimizing a certain distance to the ideal diversity distributions.}



 %, which differs from subset selection as in multiwinner elections.  
%Finally, Bredereck \etal \cite{bredereck2018multiwinner} and Celis, Huang \etal \cite{celis2017multiwinner} use diversity constraints in multiwinner elections, which can cause unfairness to smaller populations. 
%Our work adds to the research that use constraints to mitigate algorithmic bias.


% Fairness notions for knapsack under multi-agent valuations have also been studied [FSTW17]. They have several approaches to aggregate voters’ preferences: individually best, diverse knapsack and fair knap- sack. The main difference is that our model ensures fairness through constraints, while their model ensures fairness through objective function. The objective function used in their model is the Nash welfare func- tion [Nas50]. The diverse knapsack model in [FSTW17] only ensures one representative item from each category, whereas our model allows different lower and upper bounds for different groups. We focus on approximation schemes for our problems, whereas [FSTW17] focused on the parameterized complexity and the complexity of the problem under some restricted special domains.
% Ajay et al. [JLN+20] study some notion of group fairness for online/offline matching problem. Their notions of fairness are similar to ours in some respect.



% \paragraph{Unconstrained Multiwinner Elections and Proportional Representation.}
% The study of the complexity of unconstrained multiwinner elections has received attention  \cite{faliszewski2017multiwinner}. Selecting a committee using Chamberlin-Courant (CC) \cite{chamberlin1983representative} rule is NP-hard \cite{procaccia2008complexity}, and approximation algorithms have resulted in the best-known ratio of $1-\frac{1}{e}$
% %is its best possible approximation ratio 
% \cite{skowron2015achieving,lu2011budgeted}. Yang and Wang~\cite{yang2018parameterized} studied its parameterized complexity. 
% %Other work also showed that d
% Another commonly studied rule, Monroe \cite{monroe1995fully}, is also NP-hard \cite{betzler2013computation, elkind2017properties}. Sonar \etal \cite{sonar2020complexity} showed that checking whether a given committee is optimal when using these two rules is hard. Finally, the hardness of problems involving restricted voter preferences and \csr have been studied   \cite{elkind2015structure,peters2017preferences} and so has the proportional representation in dynamic ranking \cite{israel2021dynamic}.

% \paragraph{Fairness in Participatory Budgeting.} Multiwinner elections are a special case of participatory budgeting, and fairness in the latter domain has also received particular attention. For example, projects (equivalent to candidates) are divided into groups and for fairness, they consider lower and upper bounds on utility
% achieved and the lower and upper bounds on the cost of projects used in every group \cite{patel2020group}. Fluschnik \etal \cite{fluschnik2019fair} aim to achieve fairness among projects using their objective function. Next, Hershkowitz \etal \cite{hershkowitz2021district} have studied fairness from the utility received by the districts (equivalent to voters), Peters \etal \cite{peters2020proportional} define axioms for proportional representation of voters, and Lackner \etal \cite{lackner2021fairness} define fairness in long-term participatory budgeting from voters' perspective. However, we note that none of these works simultaneously consider fairness from the perspective of both, the projects and the districts. 




Overall, the work by Bredereck \etal \shortcite{bredereck2018multiwinner}, Celis \etal \shortcite{celis2017multiwinner}, Relia \shortcite{relia2021dire}, Suhr \etal \shortcite{suhr2019two}, and Yang \etal \shortcite{yang2019balanced} is closest to ours but we differ as we: (i) propose a model that can fairly allocate fairness in varying contexts, and (ii) consider the consequence of enforcing fairness on one or more actors of the system to one main actor of a single-sided platform. Additionally, our work also differs from Conitzer \etal \shortcite{conitzer2019group} as we use predefined populations and use each population's collective preferences. %Additionally, no previous work, to the best of our knowledge, has considered fairness from the perspective of voter attributes.% or has delineated candidate and voter attributes even when they coincide.


==> FairlyFairMWE - arXiv-4/preamble.tex <==
\usepackage{times}
\renewcommand*\ttdefault{txtt}
\usepackage{soul}
\usepackage{url}
%\usepackage[hidelinks]{hyperref}
\usepackage[utf8]{inputenc}
%\usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{booktabs}
%\usepackage{algorithm}
%\usepackage{natbib}
%\usepackage{algorithmic}
%\usepackage{algorithmicx}
\urlstyle{same}


%begin: custom commands and packages{
%\usepackage{amssymb}
\usepackage{subcaption}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{footnote}
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\julia}[1]{\textcolor{blue}{[Julia: #1]}}
\newcommand{\jf}[1]{\footnote{\textcolor{blue}{[Julia: #1]}}}
\newcommand{\kunal}[1]{[\textcolor{red}{{\bf Kunal: }#1}]}

\newcommand{\pe}{\emph{preference elicitation}\xspace}
\newcommand{\va}{\emph{scoring and aggregation}\xspace}
\newcommand{\cs}{\emph{committee selection}\xspace}
\newcommand{\csr}{committee selection rule\xspace}
\newcommand{\csrs}{committee selection rules\xspace}
\newcommand{\sr}{selection rule\xspace}
\newcommand{\UCWD}{UCWD\xspace}
\newcommand{\DiReCF}{DRCF\xspace}
\newcommand{\DiReCFp}[2]{DRCF\xspace}
\newcommand{\DiReCWD}{DRCWD\xspace}
\newcommand{\DiReCWDp}[2]{DRCWD\xspace}
\newcommand{\DiReCWDpse}[2]{DRCWD\xspace}
\newcommand{\DiReCWDpsu}[2]{DRCWD\xspace}
\newcommand{\DiRe}{DiRe\xspace}
\newcommand{\DIRE}{DiRe\xspace}
\newcommand{\group}[2]{A_{(#1, #2)}}
\newcommand{\groupsub}[2]{A_{(#1, #2_#1)}}
\newcommand{\population}[2]{P_{(#1, #2)}}
\newcommand{\populationsub}[2]{P_{(#1, #2_#1)}}
\newcommand{\nphard}{NP-hard\xspace}
\newcommand{\nphardshort}{NP-h\xspace}



\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\etc}{etc.\xspace}
\newcommand{\wrt}{w.r.t.\xspace}
\newcommand{\etal}{\emph{et~al.}\xspace}
%\renewcommand{\paragraph}[1]{\vspace{.2cm} \noindent \textbf{#1.}}
\usepackage{amsthm}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\usepackage{multirow}
\usepackage{xfrac}
\usepackage{subcaption}
\usepackage{balance}
\usepackage[switch]{lineno} %
%\usepackage[noend]{algorithmic}
%\usepackage{adjustbox}

\usepackage{imakeidx}
\usepackage{mathtools}
%\usepackage{algpseudocode}

\DeclareMathOperator{\pos}{pos}
\DeclareMathOperator{\CC}{CC}
\DeclareMathOperator{\score}{score}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\WU}{WU}
\DeclareMathOperator{\U}{U}
\DeclareMathOperator{\Borda}{Borda}


==> new_tex/model+complexity.tex <==
\section{Fairly Allocating Fairness}
\label{sec:Model}

In this section, we formally define a model that maps the \DIRE Committee Winner Determination problem to a problem of fairly allocating indivisible goods. The model mitigates unfairness to the voter population caused by \DIRE Committees. We first define constraints. 

\paragraph{Diversity Constraints,} denoted by $l^D_G \in [1,$ $\min(k, |G|)]$ %\ideally will be better if it is min(k, |G|)
for each candidate group $G \in \mathcal{G}$, enforces at least $l^D_G$ candidates from the group $G$ to be in the committee $W$. Formally,  $\forall$ $G \in \mathcal{G}$, $|G \cap W|\geq l^D_G$. 
%\julia{What's $D$ and why do you need it?  R is also a voting rule.  I wouldn't use D or R; attributes are attributes, if it's for candidates - you call that diversity, if it's for voters - you call that representation.}\kunal{I'll remove it from the attributes. But, we will need it to identify the 2 different types of constraints. I'll change the notation for scoring rule.} \julia{Too late to change now probably, but this is very non-standard notation. What you have here are categorical attributes; each categorical attribute has a cardinality (the number of values); each attribute partitions the candidates or the voters.}
%We note that we do not propose to use the upper bounds as it induces quota system, which is not desirable from social choice perspective. 

%\vspace{-0.15cm}
\paragraph{Representation Constraints,} denoted by $l^R_P \in [1,k]$ for each voter population $P \in \mathcal{P}$, enforces at least $l^R_P$ candidates from the population $P$'s committee $W_P$ to be in the committee $W$. Formally,  $\forall$ $P \in \mathcal{P}$, $|W_P \cap W|\geq l^R_P$.

\begin{definition}
\label{def-DiReCWD}
\textbf{($\mu,\pi$, $\mathtt{f}$)-\DIRE Committee Winner Determination (\DiReCWD):}  We are given an instance of election $E=(C,V)$,  
%set $C$ of $m$ candidates, a set $V$ of $n$ voters such that each voter $v \in V$ has a preference list $\succ_{v}$ over $m$ candidates, 
a committee size $k \in [m]$, a set of candidate groups $\mathcal{G}$ under $\mu$ attributes and their diversity constraints $l^D_G$  $\forall$ $G \in \mathcal{G}$, a set of voter populations $\mathcal{P}$ under $\pi$ attributes and their representation constraints $l^R_P$ and the winning committees $W_P$  $\forall$ $P \in \mathcal{P}$, and a \csr $\mathtt{f}$.
Let $\mathcal{W}$ denote the family of all size-$k$ committees. 
The goal of \DiReCWD is to select committees $W \in \mathcal{W}$ that satisfy  diversity and representation constraints such that $|G\cap W|\geq l^D_G$  $\forall$ $G\in \mathcal{G}$ and $|W_P\cap W|\geq l^R_P$  $\forall$ $P\in \mathcal{P}$ and maximizes, $\forall W \in \mathcal{W}$, $\mathtt{f}(W)$. Committees that satisfy the constraints are \DiRe committees.
\end{definition}


Example~\ref{eg-balanced} showed that a \DiRe committee may create or propagate biases by systematically increasing the selection of lower preferred candidates. This may result in more loss in utility to historically disadvantaged, smaller voter populations.

To mitigate this, we model our problem of selecting a committee as allocating goods (candidates) into $k$ slots. Hence, to assess the quality of candidates being selected from voter populations, we borrow ideas from the literature on the problem of fair resource allocation of indivisible goods \cite{brandt2016handbook}. Formally, given a set of $n$ agents, a set of $m$ resources, and a valuation each agent gives to each resource, the problem of fair allocation is to partition the resources among agents such that the allocation is fair. There are three classic fairness desiderata, namely, proportionality, envy-freeness, and equitability \cite{freemanrecent}. Intuitively, proportionality requires that each agent should receive her ``fair share'' of the utility, envy-freeness requires no agent should wish to swap her allocation with another agent, and equitability requires all agents should have the exact same value for their allocations and no agent should be jealous of what another agent receives. As balancing the loss in utility to candidate groups is analogous to balancing the fairness in ranking \cite{yang2019balanced}, we focus on balancing the loss in utility to voter populations. We propose varying notions of envyfreeness to balance the loss in utility to voter populations\footnote{Our model, \emph{Fairly Allocating} Fairness in Multiwinner Elections, is analogous to a Swiss Army knife. If not as useful as the knife, it can be applicable to more or less any context of a constrained multiwinner election, and the setting of the model can be chosen based on the context.}:


\subsection{Favorite-Envyfree-Committee (FEC)} Each population deserves their top-ranked candidate to be selected in the winning committee. However, selecting a \DiRe committee may result into an imbalance in the candidates selected from each population's ranking. A natural relation of FEC is finding a committee with a bounded level of envy. Specifically, we allow top $x$ ranked in the committee where $x \in [k]$. We call this relaxation FEC up to $x$.
%All proofs are included in the Appendix.

\begin{theorem}\label{thm:FECuptoxP}
Given a \DIRE Committee, there is a polynomial time algorithm that determines whether W', a FEC up to $x$, $\forall x \in \{0,$ $k-2,$ $k-1\}$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{algorithm}[ht!]
\caption{FEC Algorithm}
\label{alg:algorithmFEC}
\begin{flushleft}
\textbf{Input}:\\
$W_P$, $\forall P \in \mathcal{P}$ - winning committee of each population\\
$l_P^R$, $\forall P \in \mathcal{P}$ - diversity constraints\\
$l_G^D$, $\forall G \in \mathcal{G}$ - representation constraints\\
$W$ - Winning \DIRE Committee\\
\textbf{Output}: True if FEC exists, False otherwise\\
\end{flushleft}
%When $x=0$:
\begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=0$}
\STATE $S$ = $\bigcup {c\in C}: \forall P \in \mathcal{P},$ $ \max_{c \in W_P} \mathtt{f}_{\Borda}^{W_P}(c)$

\STATE \textbf{if} $|S|>k$ \textbf{then} \textbf{return} {False}
\STATE \textbf{if} $S\subseteq W$ and  $|S|>0$ \textbf{then} \textbf{return} {True}
\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \cap S|<l_G^D$ \textbf{then} \textbf{return} {False}
\ENDFOR
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $|W_P \cap S|<l_P^R$ \textbf{then} \textbf{return} {False}
\ENDFOR
\STATE \textbf{return} {True}
\ENDIF
% \end{algorithmic}
% %When $x= k-1$:
% \begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=k-1$}
\STATE \textbf{return} {True}
\ENDIF
% \end{algorithmic}
% %When $x=k-2$:
% \begin{algorithmic}[1] %[1] enables line numbers
\IF{$x=k-2$}
\STATE $S$ = $\phi$

\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE $S$ = $W \setminus$ $\{\forall c \in W_P : c$ is the lowest scoring candidate $\mathtt{f}_{\Borda}^{W_P}(c)$ among $W_P\}$
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $|W_P \cap S|<l_P^R$ \textbf{then} \textbf{return} {False}
\ENDFOR

\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \cap S|<l_G^D$ \textbf{then} \textbf{return} {False}
\ENDFOR
\ENDFOR
\STATE \textbf{return} {True}
\ENDIF
\end{algorithmic}
\end{algorithm}


\begin{proof}
Algorithm~\ref{alg:algorithmFEC} clearly runs in time polynomial of the size of input. For correctness, consider the following cases:

\begin{itemize}
    \item \textbf{When $\mathbf{x=0}$}, FEC up to 0 can only exist if $\forall P \in \mathcal{P}$, the population top-scoring candidate $\mathtt{f}_{\Borda}^{W_P}(c)$ is in the committee. Hence, we select each and every top-ranked candidate into set $S$. Then, if set $S$ satisfies all the given constraints, then we know FEC up to 0 exists.
    \item \textbf{When $\mathbf{x=k-1}$}, then existence of a \DiRe committee implies existence of FEC as FEC up to $k-1$ is equivalent to satisfying the requirement that each population has at least one candidate in the committee, which is in line with the definition of the \DiRe committees.
    \item \textbf{When $\mathbf{x=k-2}$}, we iterate over each population $P \in \mathcal{P}$ such that we remove the population's winning committee's $W_P$ least favorite candidate. If the candidates that remain in $W$ satisfy all the constraints after removal of this candidate, then it implies that FEC up to $k-2$ exists. This is because if a \DiRe committee exists even after removing a population's least favorite candidate, then it implies that FEC up to $k-2$ also exists. 
\end{itemize}

\end{proof}

Note that the above theorem encompasses hardness\footnote{The hardness results throughout the paper are under the assumption P $\neq$ NP.} for FEC and FEC up to $x$ as FEC and FEC up to $x$ when $x=0$ are equivalent. 

\begin{theorem}\label{thm:FECuptoxNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a FEC up to $x$, $\forall x \in [1,$ $k-3]$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{proof}
We give a reduction from vertex cover problem on $y$-uniform hypergraphs \cite{garey1979computers} to FEC up to $z$. 

An instance of vertex cover problem on $y$-uniform hypergraphs consists of a set of vertices $X$ = $\{x_1,x_2,\dots,x_{m}\}$ and a set of $|\mathcal{P}|$ hyperedges $S$, each connecting exactly $y$ vertices from $X$. A vertex cover $X' \subseteq X$ is a subset of vertices such that each edge contains at least one vertex from $X$ (i.e. $s\cap X'\neq\phi$ for each edge $s\in S$). The vertex cover problem on $y$-uniform hypergraphs is to find a vertex cover $X'$ of size at most $d$. 

We construct the FEC up to $z$ instance as follows. For each vertex $x \in X$, we have the candidate $c \in C$. For each edge $s \in S$, we have $z+1$ most favorite candidates for each $P \in \mathcal{P}$. Note that we have $|\mathcal{P}|=|S|$. In FEC up to $z$, the requirement is that at least one of the top $z+1$ candidates from each population should be in the committee. Satisfying this requirement ensures that each population is mutually envyfree up to $z$ candidates. Thus, we set $z$ = $y-1$. This corresponds to the requirement that $s\cap X'\neq\phi$. 

Hence, we have a vertex cover $X'$ of size at most $d$  if and only if we have a FEC up to $z$ committee $W$ of size at most $d$ that satisfies the requirement that at least one of the top $z+1$ candidate is in the committee, for all $P \in \mathcal{P}$. 

Note that this reduction holds $\forall z \in [1,$ $k-3]$. 
\end{proof}





\subsection{Utility-Envyfree-Committee (UEC)} Each population deserves to minimize the difference between the utilities each one gets from the selected winning committee, where the utility is the sum of Borda scores that the population gives to the candidates in the winning committee. However, a \DiRe committee may result into an unequal utility amongst all the populations. Formally, for each $P \in \mathcal{P}$, the utility that the population gets from a winning \DiRe committee $W$ is:
    \[ \U_P = \sum_{c \in  W} \mathtt{f}_{\Borda}^{W_P}(c) \]
where $\mathtt{f}_{Borda}^{W_P}(c)$ is the Borda score that candidate $c$ gets based on its rank in population $P$'s winning committee $W_P$. Overall, a UEC is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) = 0 \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| = 0 \]

%\vspace{0.2cm}
\begin{theorem}\label{thm:UECNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a UEC, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{proof}
We give a reduction from the subset sum problem \cite{garey1979computers} to UEC. An instance of subset sum problem consists of a set of non-negative integers $X$ = $\{x_1,x_2,\dots,x_{m}\}$ and a non-negative integer $sum$. The subset sum problem is to determine if there is a subset of the given set with sum equal to given $sum$.  


We construct the UEC instance as follows. We have $|X|$ candidates, which equals to $m$ candidates. Next, we have a $m$-sized scoring vector $\mathbf{s}=\{s_1, s_2, \dots, s_m\}$ such that each $s_i \in \mathbf{s}$ corresponds to $x_i \in X$ sorted in non-increasing order based on the values. Next, we have two population $P$ and $P'$ with $l_P^R= l_{P'}^R$ and let the total utility that population $P$ gets be equal to $sum$. The utility that $P'$ gets from each candidate $c$ depends on the position of $\pos_P(c)$ such that $s_1$ is the utility for candidate on position one, $s_2$ is the utility for candidate on position two, and so on. In UEC, the requirement is that the utility that $P$ gets from a committee $W$ should be the same as the utility $P'$ gets from $W$. Satisfying this requirement ensures that both populations are mutually envyfree. This implies that the total utility that population $P'$ gets from $W$ should be equal to $sum$. This corresponds to the requirement that there is a subset of the given set with sum equal to given $sum$. 

Hence, we have a subset sum if and only if we have a UEC $W$ giving a utility of $sum$ to population $P'$ and $P$.
\end{proof}

A natural relaxation of UEC is UEC up to $\eta$ where $\eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2}]$. This is to say that each population deserves to minimize the difference between utilities from the selected winning committee but up to $\eta$. Hence, a UEC  up to $\eta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|, \eta) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) \leq \eta \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| \leq \eta \]
%\vspace{0.1cm}
\begin{corollary}\label{thm:UECuptoetaNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a UEC up to $\eta$, $\forall \eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2})$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}
    
Note that when $\eta=0$, UEC up to $\eta$ and UEC are equivalent. When $\eta=\frac{(m-1)\cdot(m)}{2}$, UEC up to $\eta$ and \DiRe committee are equivalent.

\begin{proof}
We know that when $\eta=0$, UEC up to $\eta$ and UEC are equivalent. Hence, given that UEC is NP-hard, UEC up to $\eta$ is also NP-hard. Moreover, our reduction in the proof of  Theorem~\ref{thm:UECNP-hard} can be slightly  modified so that it holds $\forall \eta \in \mathbb{Z}: \eta \in \bigl[0,$ $\frac{(m-1)\cdot(m)}{2}\bigr)$. More specifically, we can reduce from subset sum where the sum is within a fixed distance from the given input $sum$ instead of subset sum.

\end{proof}
    
\subsection{Weighted-Envyfree-Committee (WEC)} Each population deserves to minimize the difference between the weighted utilities they get from the selected winning committee. The weighted utility is the sum of Borda scores that the population gives to the candidates in the winning committee who are among their top-$k$ candidates over the maximum Borda score that they can give to candidates based on their representation constraint. Formally, for each $P \in \mathcal{P}$, the weighted utility that the population having representation constraint $l_P^R$ gets from a winning \DiRe committee $W$ is:
    \[ \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \]

Overall, a WEC is a $k$-sized committee such that it aims to

%\[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|) \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| = 0 \]


%\vspace{0.1cm}
\begin{theorem}\label{thm:WECNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a WEC, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{theorem}

\begin{proof}
We give a reduction from the subset sum problem \cite{garey1979computers} to WEC. An instance of subset sum problem consists of a set of non-negative integers $X$ = $\{x_1,x_2,\dots,x_{m}\}$ and a non-negative integer $sum$. The subset sum problem is to determine if there is a subset of the given set with sum equal to given $sum$.  


We construct the WEC instance as follows. We have $|X|$ candidates, which equals to $m$ candidates. Next, we have a $m$-sized scoring vector $\mathbf{s}=\{s_1, s_2, \dots, s_m\}$ such that each $s_i \in \mathbf{s}$ corresponds to $x_i \in X$ sorted in non-increasing order based on the values. Next, we have two population $P$ and $P'$ such that $l_P^R= l_{P'}^R$, $W_P \cap W_{P'} \neq \phi$, and $\{\{W_P \cup W_{P'}\} \setminus \{W_P \cap W_{P'}\}\} \cap W = \phi $. Let the total utility that population $P$ gets be equal to $sum$. Hence, the weighted utility will be 
\[   \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \leq \frac{\sum_{c \in W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{m}m-i} \]

Next, the $sum$ can be written as

\[sum =  \sum_{c \in W} \mathtt{f}_{\Borda}^{W_P}(c)\]

Hence, 
\[    \frac{\sum_{c \in W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{m}m-i} \leq sum  \]

Therefore, \[   \WU_P \leq sum \]



The utility that $P'$ gets from each candidate $c$ depends on the position of $\pos_P(c)$ such that $s_1$ is the utility for candidate on position one, $s_2$ is the utility for candidate on position two, and so on. In WEC, the requirement is that the weighted utility that $P$ gets from a committee $W$ should be the same as the weighted utility $P'$ gets from $W$. Satisfying this requirement ensures that both populations are mutually envyfree. This implies that the total utility that population $P'$ gets from $W$ should be equal to 

\[   \WU_{P'} = \frac{\sum_{c \in W_{P'} \cap W} \mathtt{f}_{\Borda}^{W_{P'}}(c)}{\sum_{i=1}^{l_{P'}^R}m-i} \]

However, as $l_P^R= l_{P'}^R$, we can rewrite $\WU_{P'}$ as 

\[   \WU_{P'} = \frac{\sum_{c \in W_{P'} \cap W} \mathtt{f}_{\Borda}^{W_{P'}}(c)}{\sum_{i=1}^{l_{P}^R}m-i} \]

Additionally, as $W_P \cap W_{P'} \neq \phi$, and $\{\{W_P \cup W_{P'}\} \setminus \{W_P \cap W_{P'}\}\} \cap W = \phi $, we know that the candidates in the winning \DiRe committee is common to both the population. Hence, 

\[\sum_{c \in W_{P'} \cap W} \mathtt{f}_{\Borda}^{W_{P'}}(c) = \sum_{c \in W_{P} \cap W} \mathtt{f}_{\Borda}^{W_{P}}(c)\]

Therefore, we can rewrite $\WU_{P'}$ as

\[   \WU_{P'} = \frac{\sum_{c \in W_{P} \cap W} \mathtt{f}_{\Borda}^{W_{P}}(c)}{\sum_{i=1}^{l_{P}^R}m-i} \]

This implies that 
\[ \WU_{P'} = \WU_{P}\]

However, for this equation to hold, it is necessary that $P'$  gets a total utility of $sum$ from $W$ in line with $P$  getting a total utility of $sum$. This corresponds to the requirement that there is a subset of the given set with sum equal to given $sum$. 

Hence, we have a subset sum if and only if we have a WEC $W$ giving a total utility of $sum$ and weighted utility of $W_P$ to population $P'$ and $P$.
\end{proof}


A natural relaxation of WEC is WEC up to $\zeta$ where $\zeta \in \mathbb{Q}: \zeta \in [0,$ $1]$. This is to say that each population deserves to minimize the difference between weighted utilities from the selected winning committee but up to $\zeta$. Hence, a WEC  up to $\zeta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|, \zeta) \]
\[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| \leq \zeta \]

\begin{corollary}\label{thm:WECuptozetaNP-hard}
Given a \DIRE Committee, it is NP-hard to determine whether W', a WEC up to $\zeta$, $\forall \zeta \in \mathbb{Q}: \zeta \in [0,$ $1)$, exists such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}

Note that when $\zeta=0$, WEC up to $\zeta$ and WEC are equivalent. When $\zeta=1$, WEC up to $\zeta$ and \DiRe committee are equivalent.
\begin{proof}
We know that when $\zeta=0$, WEC up to $\zeta$ and WEC are equivalent. Hence, given that WEC is NP-hard, WEC up to $\zeta$ is also NP-hard. Moreover, our reduction in the proof of  Theorem~\ref{thm:WECNP-hard} can be slightly  modified so that it holds $\forall \zeta \in \mathbb{Q}: \zeta \in [0,$ $1)$. More specifically, we can reduce from subset sum where the sum is within a fixed distance from the given input $sum$ instead of subset sum. $\zeta$ will be a function of this distance and $\forall P \in \mathcal{P}$, $|W_P\cap W|$ and $l_P^R$.

\end{proof}

\subsection{Localized Fair Allocation}

Specifically, we say that an allocation is locally envy-free if no agent envies a neighbor’s allocation and locally proportional if each agent values her own allocation as much as the average value of her neighbor’s allocations, with the former implying the latter. While global envy-freeness implies local envy-freeness, global proportionality does not imply local proportionaity, or vice versa. A general result is that for any two distinct graphs on the same set of nodes and an allocation, there exists a set of valuation functions such that the allocation is locally proportional on one but not the other.




\section{Mitigating Manipulation in \DIRE Elections}

Another unintended consequence and cause of unfairness in \DiRe committees is that it easily allows manipulation\footnote{
All voting mechanisms are known to be susceptible to manipulation \cite{gibbard1973manipulation}, i.e., a situation when a strategizing voter or a group of voters misrepresents his preferences in order to obtain a more desirable outcome. See \cite{elkind2005hybrid} for details.} of outcomes by larger populations to adversely impact smaller, under-represented population. For example, assume Californian voters in Figure~\ref{fig:whatexample/voters} are already manipulated. This is to say that had the California voters \emph{not} swapped position of $c_5$ and $c_6$, then Illinois' most preferred candidate $c_5$ would have been part of the \DiRe committee implicitly. However, the votes are manipulated by changing the preferences among the non-top-$k$ candidates preferred by the Californian voters. This resulted in an adverse outcome for Illinois, without affecting California (see Example~\ref{eg-balanced}).  

\begin{theorem}\label{thm:DiReManipulation-easy}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then there is a polynomial time algorithm that can either help some manipulator population $P \in \mathcal{P}$ manipulate \DiReCWD or determine that \DiReCWD is not manipulable as long as $P$ satisfies the following conditions:
\begin{itemize}
    \item $|P|>|P'|$, $\forall P' \in \mathcal{P}$
    \item $P$ swaps preferences within $C \setminus W_P$
\end{itemize}
\end{theorem}

\begin{algorithm}[ht!]
\caption{\DiReCWD Manipulation Algorithm}
\label{alg:algorithmManipulation}
\begin{flushleft}
\textbf{Input}:\\
$W_P$, $\forall P \in \mathcal{P}$ - winning committee of each population\\
$l_P^R$, $\forall P \in \mathcal{P}$ - diversity constraints\\
$l_G^D$, $\forall G \in \mathcal{G}$ - representation constraints\\
$W$ - Winning \DIRE Committee\\
\textbf{Output}: Manipulated votes if manipulation possible, False otherwise\\
\end{flushleft}

\begin{algorithmic}[1] %[1] enables line numbers
\STATE $P_{\max}$ = $P \in \mathcal{P}:\max(|P|)$
\STATE $E_{\text{actual}}$ = Store the actual votes and $W_P$, $\forall P \in \mathcal{P}$ of election $E$

\FOR{\textbf{each} $c \in C \setminus W_{P_{\max}}$}
\FOR{\textbf{each} $c' \in C \setminus W_{P_{\max}} \setminus c$}
\STATE swap $\pos_v(c)$ and $\pos_v(c')$ for all $v\in P_{\max}$
\STATE $E_{\text{manip}}$ = Store the manipulated votes and corresponding $W_P$,  $\forall P \in \mathcal{P}$ of election $E$
\FOR{\textbf{each} $P \in \mathcal{P}$}
\STATE \textbf{if} $W_P \in E_{\text{actual}} \neq W_P \in E_{\text{manip}}$ and $|W_P \in E_{\text{manip}} \cap W\in E_{\text{manip}}|<l_P^R$ \textbf{then} \textbf{return} Maipulated Election $E_{\text{manip}}$
\ENDFOR
\FOR{\textbf{each} $G \in \mathcal{G}$}
\STATE \textbf{if} $|G \in E_{\text{manip}} \cap W\in E_{\text{manip}}|<l_G^D$ \textbf{then} \textbf{return} Maipulated Election $E_{\text{manip}}$
\ENDFOR
\STATE swap $\pos_v(c)$ and $\pos_v(c')$ for all $v\in P_{\max}$
\ENDFOR
\ENDFOR
\STATE \textbf{return} {False}
\end{algorithmic}
\end{algorithm}
\begin{proof}
Algorithm~\ref{alg:algorithmManipulation} clearly runs in time polynomial of the size of input. Note that as $\mathtt{f}$ is a monotone, separable scoring function, we know that 
\[\mathtt{f}(W)=\sum_{c\in W}\mathtt{(c)}\] 
Hence, it implies that computing $W_P$, $\forall P \in \mathcal{P}$ and $W$ for each of the manipulated instance of the election takes polynomial time. For correctness, it is easy to see that the largest population exhaustively swaps each of its bottom $m-k$ candidates and compares the change in outcome. If the outcome changes for any other population or candidate group, then manipulation is successful. Otherwise, the algorithm terminates by returning False.

Note that the algorithm can be easily modified to assess if \emph{any} population can manipulate the election. Instead of choosing the largest population in Line 1 of the algorithm, we can have a For loop that iterates over each population and check whether they can manipulate the result or not.
\end{proof}


For the last theorem, note that the NP-hardness of finding a \DiRe committee does \emph{not} follow and result into NP-hardness of manipulating \DiRe committee elections. This is because we assume that a \DiRe committee is given as an input. In contrast, the next three proofs show that even when \DiRe committees are given, using FEC, UEC, or WEC makes it hard to manipulate \DiRe committee elections. Thus, the models proposed in this paper also mitigate an unintended consequence of imparting fairness (Diversity and Representation constraints) in elections, the consequence being the ease to manipulate elections.


Promisingly, our model has an advantage that even the easiest version of each of the envyfreeness models makes the \DiRe committee selection problem resistant to manipulation. In principle, this is because swapping non-top-$k$ preferences by Californian voters penalizes them as well.


\begin{corollary}\label{thm:DiReManipulationFEC-hard}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a FEC, such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}

\begin{proof}
Theorem~\ref{thm:FECuptoxNP-hard} showed that finding a FEC is NP-hard. Hence, if finding FEC in a regular election is NP-hard, then the hardness of manipulating FEC election follows the hardness of finding a FEC.
\end{proof}
%\vspace{0.1cm}
\begin{corollary}\label{thm:DiReManipulationUEC-hard}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a UEC, such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}
\begin{proof}
Theorem~\ref{thm:UECNP-hard} showed that finding a UEC is NP-hard. Hence, if finding UEC in a regular election is NP-hard, then the hardness of manipulating UEC election follows the hardness of finding a UEC.
\end{proof}
%\vspace{0.1cm}
\begin{corollary}\label{thm:DiReManipulationWEC-hard}
If $\mathtt{f}$ is a monotone, separable scoring function and given a \DiRe committee, then it is NP-hard for any manipulator population $P \in \mathcal{P}$ to manipulate election of $W'$, a WEC, such that $\forall G \in \mathcal{G}, G \cap W' \geq l^D_G$ and $\forall P \in \mathcal{P}, W_P \cap W' \geq l^R_P$.
\end{corollary}

\begin{proof}
Theorem~\ref{thm:WECNP-hard} showed that finding a WEC is NP-hard. Hence, if finding WEC in a regular election is NP-hard, then the hardness of manipulating WEC election follows the hardness of finding a WEC.
\end{proof}

In summary, while mitigating utility-based unfairness caused due to fairness is generally hard, our models make causing manipulation-based unfairness hard as well. The latter intractability is desirable.

%In summary, we deem these proposed notions of envyfreeness among voter populations to be of interest, especially due to the promising empirical results that we got from our initial analysis (discussed in the next section). We also plan to study the theoretical aspects of these notions.
